Graph Analytics on Evolving Data (Abstract)

We consider the problem of graph analytics on evolving graphs. In this scenario, a query typically needs to be applied to different snapshots of the graph over an extended time window. We propose CommonGraph, an approach for efficient processing of queries on evolving graphs. We first observe that edge deletions are significantly more expensive than addition operations. CommonGraph converts all deletions to additions by finding a common graph that exists across all snapshots. After computing the query on this graph, to reach any snapshot, we simply need to add the missing edges and incrementally update the query results. CommonGraph also allows sharing of common additions among snapshots that require them, and breaks the sequential dependency inherent in the traditional streaming approach where snapshots are processed in sequence, enabling additional opportunities for parallelism. We incorporate the CommonGraph approach by extending the KickStarter streaming framework. CommonGraph achieves 1.38x-8.17x improvement in performance over Kickstarter across multiple benchmarks.

==> algo-first.tex <==
\begin{algorithm*}[!t]
\begin{multicols}{2}
\begin{algorithmic}[1]

\State{\textbf{Inputs}: Snapshots; Additions; and Deletions.}
\State{Snapshots-- $G_1(V_1,E_1)$, $G_2(V_2,E_2)$, ... , $G_N(V_N,E_N)$; \\
Batches of Additions -- $\Delta_{G_1}^+$, $\Delta_{G_2}^+$, ... , $\Delta_{G_N}^+$; \\
Batches of Deletions -- $\Delta_{G_1}^-$, $\Delta_{G_2}^-$, ... , $\Delta_{G_N}^-$;}
\State{\textbf{Output}: $TG\;$ \& $\;Tree$ (Minimum Cost Schedule).}
\Statex{}
%\State{\textcolor{red}{$\rhd$ Creating CommonGraph Tree:}}
\State{\textsc{Build-Triangular-Grid;}}
%\State{\textcolor{red}{$\rhd$ Finding the best Paths with Minimum Cost using the Steiner Tree Algorithm}}
\State{\textsc{Identify-Steiner-Tree; }}
%\State{\textcolor{red}{$\rhd$ Combining the Addition Lists}}
\State{\textsc{Compress-Steiner-Tree; }}
\Statex{}
  
\Function{Build-Triangular-Grid }{}
\State{$S \leftarrow$ Snapshots; $\;\;\;TG \leftarrow \phi$; $\;\;\;i \leftarrow 0$;}
\For{each $G_i(V_i,E_i)$ and $G_{i+1}(V_{i+1},E_{i+1})$ $\in S$}
\If{$G_i$ and $G_{i+1}$ are leaf nodes}
\State{$w_1 = \Delta_{G_{i}}^-$; $\;\;\;w_2 = \Delta_{G_{i}}^+$}
\Else
\State{$w_1 = \Delta_{G_{i+1}}^- - \Delta_{G_{i}}^+$; \;\;\;$w_2 = \Delta_{G_{i}}^+ - \Delta_{G_{i+1}}^-$;}
\State{$\Delta_{ICG_{i}}^+ = w_2$; $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\Delta_{ICG_{i}}^- = w_1$}
\EndIf
\State{$TG \leftarrow TG \cup \{(ICG_{i}, G_i, w_1)$}
\State{$TG \leftarrow TG \cup \{(ICG_{i}, G_{i+1}, w_2)$}
\State{$S \leftarrow S \cup ICG_{i}$; $\;\;\;\;i \leftarrow i + 1$}
\EndFor
\EndFunction
\Statex{}

\Statex{}
\Function{Identify-Steiner-Tree }{}
\State{Let $Terminals$ be the leaves and root in $TG$;}
\State{$Tree \leftarrow$ subtree of $TG$ with at least one terminal;}
\While{$Tree$ does not span all terminals}
\State{Select a terminal $x$ not in $Tree$ such that}
\State{ $\;\;\;\;x$ is closest to a vertex in $Tree$}
\State{Add to $Tree$, shortest path connecting $x$ to $Tree$}
\EndWhile
\EndFunction
\Statex{}

\Statex{}
\Function{Compress-Steiner-Tree }{}
\For{each vertex $v \in Tree$}
\If{$v$ has one incoming and one outgoing edge}
%\State{\textsc{Remove} $(v)$}
\State{\textsc{Bypass} $v$}
\EndIf
\EndFor
\EndFunction
\Statex{}
\Statex{}
\Statex{}
\Statex{}
\end{algorithmic}
\end{multicols}
\caption{Algorithm for Identifying Minimum Cost Query Evaluation Schedule using the Steiner Tree Algorithm.}\label{algo:tree_construction}
\end{algorithm*}

==> algorithm.tex <==
\section{CommonGraph Algorithms}\label{section3}
We present two \textit{CommonGraph} based algorithms for evaluating a query on a sequence of snapshots corresponding to a time window. First, we present the \emph{direct hop} algorithm for query evaluation and show the work sharing enabled by the \emph{CommonGraph} reduces the cost of query evaluation. Second, we present the \emph{Triangular Grid} (TG) representation, which provides \textit{CommonGraph} representations for subsequences of snapshots, and show how it is used to find an even better query evaluation schedule that maximizes work sharing.

%\subsection{Two Snapshots}
%The simplest scenario in the evolving graph is when we have two snapshots. As shown in the fig.~\ref{fig:common_graph_example}, assume we have two snapshots of a graph in different points named $G_i$ and $G_{i+1}$, respectively. These two snapshots are already available, and both contain all the same vertices. We will reach $G_{i+1}$ by adding $\Delta^{i}_+$ edges to $G_i$ and removing $\Delta^{i}_-$ edges from it. In \textit{CommonGraph} algorithm we will combine \textit{concurrency} with incremental processing that involves only additions. As shown in fig.~\ref{fig:common_graph_example}, first we will evaluate the query on $G_c$ and then we will concurrently update the results for $G_i$ and $G_{i+1}$ by applying $\Delta^{i}_-$ and $\Delta^{i}_+$ additions respectively. $G_c$ contains the edges, which are present in both in $G_i$ and $G_{i+1}$. Therefore, $G_c$ is the intersection of both $G_i$ and $G_{i+1}$. Since the $G_c$ is the intersection of $G_i$ and $G_{i+1}$, we can simply derive $G_i$ and $G_{i+1}$ by applying $\Delta^{i}_-$  and $\Delta^{i}_+$ to $G_c$, respectively. Therefore, we can conclude that $\Delta^{c(i)}_+$ $=$ $\Delta^{i}_-$ and $\Delta^{c(i+1)}_+$ $=$ $\Delta^{i}_+$. In the example in fig.~\ref{fig:common_graph_example}, $\Delta^{i}_+$ contains three edges $\{e3, e12, e15\}$, and $\Delta^{i}_-$ contains five edges $\{e9, e11, e16, e23, e29\}$. Therefore, we need to add five additions to reach from $G_c$ to $G_i$ and we need to add 3 three additions to reach from $G_c$ to $G_{i+1}$. Using this idea, we completely removed deletion and only have additions in this scenario.     

%Based on the motivation data we saw in the previous sections, the cost of the deletion is roughly four times bigger than the cost of the addition. Therefore, if we assume the cost of each addition to be \textit{x}, then the cost of each deletion will be 4\textit{x}. In our example in fig.~\ref{fig:common_graph_example}, the $\Delta^{i}_+$ deletion batch contains 5 edges and $\Delta^{i}_+$ addition batch contains the 3 edges. Therefore, we have five deletions and three additions; thus, the total cost of the basic scenario is $(4x\times5)+3x=18x$, but if we use the \textit{addition-only} scenario, we need to apply five additions to go from $G_c$ to $G_i$ and we should have three additions to go from $G_c$ to $G_{i+1}$. The cost of each addition is \textit{x}; therefore, the total cost of this scenario is 8\textit{x}, which is considerably less than the total cost of the basic scenario.

\subsection{Direct Hop Query Evaluation}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\columnwidth]{diagrams/direct-hop.pdf}
    \caption{Showing an example for direct-hop algorithm.}
    \label{fig:direct-hop}
    \vspace{-0.15in}
\end{figure}

Since the \emph{CommonGraph} represents edges common to all snapshots under consideration, a significant degree of \emph{work sharing} across snapshots is achieved by evaluating the query on the \emph{CommonGraph} and then updating the results incrementally by applying the impact of edge additions corresponding to each snapshot. This approach avoids the need to use the expensive incremental algorithm for deletions while achieving significant work sharing via the \emph{CommonGraph}. We name this method the \emph{direct-hop} algorithm because the query evaluation schedule directly computes the query results for each snapshot from the results of the \emph{CommonGraph}.

The example in Figure~\ref{fig:direct-hop} illustrates the benefits of this approach. Let us consider we have three snapshots namely $G_i$, $G_{i+1}$, and $G_{i+2}$. Let us assume that the batches of edge additions and deletions that derive $G_{i+1}$ from $G_i$ (i.e., $\Delta^{i}_+$ and $\Delta^{i}_-$) and then derive $G_{i+2}$ from $G_{i+1}$ (i.e., $\Delta^{i+1}_+$ and $\Delta^{i+1}_-$) are as shown in Figure~\ref{fig:direct-hop}.

%given below: 
%\hspace{0.5in}
%\begin{tabular}{l}
%$\Delta^{i}_+ \:\;\;=\; \{e3, e12, e15\}$ \\
%$\Delta^{i}_- \:\;\;=\; \{e9, e11, e16, e23, e29\}$ \\
%$\Delta^{i+1}_+ =\; \{e9, e11, e14, e24, e29\}$ \\
%$\Delta^{i+1}_- =\; \{e3, e4, e7, e10, e26\}$ \\
%\end{tabular}
%\vspace{0.05in}

Consider that the \textit{CommonGraph} $G_c$ that has all the common edges from the three snapshots as shown in Figure~\ref{fig:direct-hop}. We can reach $G_i$, $G_{i+1}$, and $G_{i+2}$ by adding $\Delta^{c1}_+$, $\Delta^{c2}_+$, and $\Delta^{c3}_+$ to $G_{c}$ respectively. Next we show that the direct-hop algorithm with only additions is more efficient than the incremental approach used in Kickstarter that evolves the graph from $G_i$ to $G_{i+1}$ to $G_{i+2}$ with both additions and deletions. Finding query results for $G_{i+1}$ from $G_i$ and $G_{i+2}$ from $G_{i+1}$ will require processing 8 additions ($|\Delta^{i}_+| + |\Delta^{i+1}_+|$) and 10 deletions ($|\Delta^{i}_-| + |\Delta^{i+1}_-|$). On the other hand, direct-hop approach will require processing of 22 additions ($|\Delta^{c1}_+| + |\Delta^{c2}_+| + |\Delta^{c3}_+|$). Since deletions are more expensive than additions (3$\times$ in Kickstarter), direct-hop evaluation is expected to be more efficient. This observation is confirmed by our experimental results presented later in the paper. Note that while Kickstarter will compute the query from scratch on $G_i$, direct-hop wil do so on the \emph{CommonGraph}. Since, the \emph{CommonGraph} is a subgraph of $G_i$, we conservatively (in favor of Kickstarter) assume that these costs are similar.

Finally, we observe that if we simply want to incrementally evaluate a query on snapshot $G_{i+1}$, then evaluating it from $G_c$ is less expensive than evaluating it from $G_i$. The former requires 7 additions and the latter requires 3 additions and 5 deletions. 

%The second scenario is when we want to find $G_{i+1}$ using the \textit{CommonGraph}. In that case, we should add seven edges to \textit{CommonGraph} to find $G_{i+1}$. Therefore, in this case, we have less number of operations, and we only have additions. Intuitively, we can say that the number of operations for finding a snapshot from \textit{CommonGraph} is less than or equal to the number of operations of the addition/deletion approach starting from the first snapshot, and we only have additions in the \textit{CommonGraph} approach. Suppose we have no common edges between the previous snapshot's addition list and the current snapshot deletion list. In that case, the number of operations in the \textit{CommonGraph} direct-hop approach is equal to the number of operations in the addition/deletion approach starting from the first snapshot. But if we have common edges between that two lists, we have fewer operations in the \textit{CommonGraph} approach. For example, in the figure, we have first added e3 and then removed $e3$; therefore, $e3$ is common, and we have one less operation in the \textit{CommonGraph} approach. 

\subsection{Triangular Grid Based Algorithm for Query Evaluation with Maximal Work Sharing}
\label{series of snapshots}
In this section we consider \emph{work sharing} when evaluating a query over a long sequence of snapshots $G_0, G_1, \cdots , G_n$. Once again $G_c$ includes all the edges that are common to all the snapshots $G_0, G_1, \cdots , G_n$ and, using the additions-only incremental algorithm, from the results of $G_c$ the results for $G_0, G_1, \cdots , G_n$ can be independently computed via direct-hop approach. However, we observe that when there are large number of snapshots, \emph{it becomes possible to create intermediate common graphs for subsequences of snapshots and take advantage of additional work sharing opportunities}.

\paragraph*{Triangular Grid:} To take advantage of additional work sharing we introduce the \emph{Triangular Grid} (TG) representation which is illustrated, without loss of generality, for three snapshots $G_i$, $G_{i+1}$, and $G_{i+2}$ in Figure~\ref{fig:multiple_snapshots_example}. The TG includes two \emph{Intermediate Common-Graphs} (ICGs) that are common-graphs for pairs of original snapshots. In Figure~\ref{fig:multiple_snapshots_example}, $G_{c(i \to i+1)}$ is the ICG for $G_i$ and $G_{i+1}$ while $G_{c(i+1 \to i+2)}$ is the ICG for $G_{i+1}$ and $G_{i+2}$. Finally, the \emph{CommonGraph} for \emph{all} three snapshots is denoted as $G_{c(i \to i+2)}$ or simply $G_c$.

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{diagrams/three-snapshots.pdf}
\captionsetup{justification=centering}
    \caption{Triagular Grid (TG) corresponding to three original snapshots $G_i$, $G_{i+1}$, and $G_{i+2}$. 
    %$G_{c1(i,i+1)}$ is the common subgraph for $G_i$ and $G_{i+1}$; $G_{c2(i+1,i+2)}$ is the common subgraph of $G_{i+1}$ and $G_{i+2}$; $G_{c(c1,c2)}$ is the common subgraph of $G_{c1(i,i+1)}$ and $G_{c2(i+1,i+2)}$ and also it is the common subgraph of our three snapshots. 
    }
    \vspace{-0.1in}\label{fig:multiple_snapshots_example}
    \vspace{-0.15in}
\end{figure}

Note that although we have shown a TG for three snapshots, the symmetric nature of the representation shows that it applies to any arbitrary number of snapshots. If there are $n$ original snapshots to be analyzed, the TG will contain exactly $n-2$ intermediate levels as the number of ICGs reduces by one for each level. More importantly we note that edges from the root \emph{CommonGraph} $G_c$ to the two ICGs and then from the two ICGs to the original snapshots are all labelled \emph{exclusively with additions}. That is, to move from the root $G_c$ to any original snapshot via intermediate ICGs we only need to perform batches of edge additions. Finally, by starting from the root $G_c$, and then potentially moving through exactly one ICG at each intermediate level, a query evaluation schedule can be chosen that exploits additional sharing among subsequence of snapshots represented by the chosen ICG.  TG guarantees the presence of an ICG to represent any consecutive sub-sequence of snapshots.  It is important to note that the ICGs are never stored and are generated on demand only by streaming the common edge additions if they are needed (that is, when we need to compute multiple snapshots reachable from the ICG).

Next we show how, from the batches of additions and deletions between original snapshots, we can compute the additions labelling all other edges in the TG leading to or originating from the ICGs. Let us assume that the batches of edge additions and deletions that derive $G_{i+1}$ from $G_i$ (i.e., $\Delta^{i}_+$ and $\Delta^{i}_-$) and then derive $G_{i+2}$ from $G_{i+1}$ (i.e., $\Delta^{i+1}_+$ and $\Delta^{i+1}_-$) are as follows: 

\hspace{0.5in}
\begin{tabular}{l}
$\Delta^{i}_+ \:\;\;=\; \{e3, e12, e15\}$ \\
$\Delta^{i}_- \:\;\;=\; \{e9, e11, e16, e23, e29\}$ \\
$\Delta^{i+1}_+ =\; \{e9, e11, e14, e24, e29\}$ \\
$\Delta^{i+1}_- =\; \{e3, e4, e7, e10, e26\}$ \\
\end{tabular}

%Therefore, we have two \textit{CommonGraphs} for three snapshots in the second level. Finally, we must compute the \textit{CommonGraph} of $G_{c1(i, i+1)}$ and $G_{c2(i+1, i+2)}$ in the third level and we name it $G_{c(c1, c2)}$. $G_{c(c1, c2)}$ contains all the common edges in our three snapshots; therefore, we can say that this is the \textit{CommonGraph} of the three snapshots. In this example, we found the CommonGraph base on a tree structure, and we can extend this tree structure to every number of snapshots. Now we know how to find the \textit{CommonGraph} for a series of snapshots, but we do not know what is our \textit{addition-only} batches to derive our multiple snapshots from a \textit{CommonGraph}. Let us again focus on fig.~\ref{fig:multiple_snapshots_example} to explain this part. By finding each addition batch for each level of the tree, we can reach from the $G_{c(c1, c2)}$ to the series of the snapshots. 
%We should compute the addition-only batches based on the $\Delta^{i}_+$, $\Delta^{i}_-$, $\Delta^{i+1}_+$, and $\Delta^{i+1}_-$.

\vspace{0.05in}
Around the intermediate level of the TG (i.e., just below the original snapshots and just above $G_c$), we can easily compute the values of the following six batches of additions corresponding to the six edges (four involving original snapshots and two involving $G_c$) as follows:

%As shown in fig.~\ref{fig:multiple_snapshots_example}, $\Delta^{c(c1)}_+$ $=$ $\Delta^{i+1}_-$ $-$ $\Delta^{i}_+$ which is equal to $\{e3, e4, e7, e10, e26\}$ $-$ $\{e3, e12, e15\}$ $=$ $\{e4, e7, e10, e26\}$ and also $\Delta^{c(c2)}_+$ $=$ $\Delta^{i}_+$ $-$ $\Delta^{i+1}_-$ which is equal to $\{e3, e12, e15\}$ $-$ $\{e3, e4, e7, e10, e26\}$ $=$ $\{e12, e15\}$. Now we have all the \textit{addition-only} batches for deriving the snapshots from $\Delta^{c(c1,c2)}_+$.
%$\Delta^{c1(i)}_+$, $\Delta^{c1(i+1)}_+$, $\Delta^{c2(i+1)}_+$, and $\Delta^{c2(i+2)}_+$. 

\vspace{0.025in}
\noindent
\begin{tabular}{l}
%\circled{1} $\;\Delta^{G_{c(i \to i+1)} \to G_i}_+ \;\;\;\;\;\;\; = \;\;\; \Delta^{i}_- \;\;\;=\;\;\; \{e9, e11, e16, e23, e29\}$ \\
\circled{1} $\;\Delta^{ICG_1 \to G_i}_+ \;\;\;\; = \;\;\; \Delta^{i}_- \;\;\;\;\;\;=\;\;\; \{e9, e11, e16, e23, e29\}$ \\
%\circled{2} $\;\Delta^{G_{c(i \to i+1)} \to G_{i+1}}_+ \;\;\;\; = \;\;\; \Delta^{i}_+ \;\;\;=\;\;\; \{e3, e12, e15\}$ \\
\circled{2} $\;\Delta^{ICG_1 \to G_{i+1}}_+ \; = \;\;\; \Delta^{i}_+ \;\;\;\;\;\;=\;\;\; \{e3, e12, e15\}$ \\
%\circled{3} $\;\Delta^{G_{c(i+1 \to i+2)} \to G_{i+1}}_+ \; = \;\;\; \Delta^{i+1}_- \;\;\;=\;\;\; \{e3, e4, e7, e10, e26\}$ \\
\circled{3} $\;\Delta^{ICG_2 \to G_{i+1}}_+ \; = \;\;\; \Delta^{i+1}_- \;\;\;=\;\;\; \{e3, e4, e7, e10, e26\}$ \\
%\circled{4} $\;\Delta^{G_{c(i+1 \to i+2)} \to G_{i+2}}_+ \; = \;\;\; \Delta^{i+1}_+ \;\;\;=\;\;\; \{e9, e11, e14, e24, e29\}$ \\
\circled{4} $\;\Delta^{ICG_2 \to G_{i+2}}_+ \; = \;\;\; \Delta^{i+1}_+ \;\;\;=\;\;\; \{e9, e11, e14, e24, e29\}$ \\
%\circled{5} $\;\Delta^{G_c \to G_{c(i \to i+1)}}_+ \;\;\;\;\;\;\; = \;\;\; \Delta^{i+1}_- \;-\; \Delta^{i}_+ \;\;\;=\;\;\; \{e4, e7, e10, e26\}$ \\
\circled{5} $\;\Delta^{G_c \to ICG_1}_+ \;\;\;\; = \;\;\; \Delta^{i+1}_- \;-\; \Delta^{i}_+ \;\;\;=\;\;\; \{e4, e7, e10, e26\}$ \\
%\circled{6} $\;\Delta^{G_c \to G_{c(i+1 \to i+2)}}_+ \;\;\; = \;\;\; \Delta^{i}_+ \;-\; \Delta^{i+1}_- \;\;\;=\;\;\; \{e12, e15\}$
\circled{6} $\;\Delta^{G_c \to ICG_2}_+ \;\;\;\; = \;\;\; \Delta^{i}_+ \;-\; \Delta^{i+1}_- \;\;\;=\;\;\; \{e12, e15\}$
\end{tabular}
\vspace{0.05in}

%As we explained in the previous section, since the \textit{CommonGraph} is the intersection of the two snapshots, if we add the $\Delta^{i}_-$ to the \textit{CommonGraph}, we can get the first snapshot, and if we add $\Delta^{i}_-$ to the \textit{CommonGraph}, we can derive the second snapshot. Therefore, the value of our addition-only batches are equal to: $\Delta^{c1(i)}_+$ = $\Delta^{i}_-$, $\Delta^{c1(i+1)}_+$ = $\Delta^{i}_+$. $\Delta^{c2(i+1)}_+$ = $\Delta^{i+1}_-$, and $\Delta^{c2(i+2)}_+$ = $\Delta^{i+1}_+$. Then we should go to the second level of the tree and compute the value of the $\Delta^{c(c1)}_+$ and $\Delta^{c(c2)}_+$. As you can see in the fig.~\ref{fig:multiple_snapshots_example}, we can find the $G_{c1(i, i+1)}$ by removing the edges in $\Delta^{i}_-$ from $G_i$. Also we can derive the $G_{i+1}$ by applying the $\Delta^{i}_+$ and $\Delta^{i}_-$ to $G_i$. Therefore, the value of $G_{i+1}$ is equal to $G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$. By removing the edges in $\Delta^{i+1}_-$ from $G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$ we can get the $G_{c2(i+1, i+2)}$ graph. Thus, $G_{c2(i+1, i+2)}$ is equal to $G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$ $-$ $\Delta^{i+1}_-$. Therefore:



\iffalse
\\
\\
$G_{c1(i, i+1)}$ $=$ $G_i$ $-$ $\Delta^{i}_-$\\
$G_{c2(i+1, i+2)}$ $=$ $G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$ $-$ $\Delta^{i+1}_-$\\
\\
We can find $\Delta^{c(c1)}_+$ by removing the edges in $G_{c1(i, i+1)}$ which are exist in $G_{c2(i+1, i+2)}$. Therefore: 
\\
\\
$\Delta^{c(c1)}_+$ $=$ $G_{c1(i, i+1)}$ $-$ $G_{c2(i+1, i+2)}$\\
$\Delta^{c(c1)}_+$ $=$ $G_i$ $-$ $\Delta^{i}_-$ $-$ ($G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$ $-$ $\Delta^{i+1}_-$)\\
\\
Therefore, the value of $\Delta^{c(c1)}_+$ is given by: \\
\\
$\Delta^{c(c1)}_+$ $=$ $\Delta^{i+1}_-$ $-$ $\Delta^{i}_+$\\
\\
We can simply find $\Delta^{c(c2)}_+$ by removing the edges in $G_{c2(i+1, i+2)}$  which exist in $G_{c1(i, i+1)}$. Therefore: 
\\
\\
$\Delta^{c(c2)}_+$ $=$ $G_{c2(i+1, i+2)}$ $-$ $G_{c1(i, i+1)}$\\
$\Delta^{c(c2)}_+$ $=$ ($G_{i}$ $+$ $\Delta^{i}_+$ $-$ $\Delta^{i}_-$ $-$ $\Delta^{i+1}_-$) $-$ ($G_i$ $-$ $\Delta^{i}_-$)\\
\\
Therefore, the value of $\Delta^{c(c2)}_+$ is given by: \\
\\
$\Delta^{c(c2)}_+$ $=$ $\Delta^{i}_+$ $-$ $\Delta^{i+1}_-$\\

As shown in fig.~\ref{fig:multiple_snapshots_example}, $\Delta^{c(c1)}_+$ $=$ $\Delta^{i+1}_-$ $-$ $\Delta^{i}_+$ which is equal to $\{e3, e4, e7, e10, e26\}$ $-$ $\{e3, e12, e15\}$ $=$ $\{e4, e7, e10, e26\}$ and also $\Delta^{c(c2)}_+$ $=$ $\Delta^{i}_+$ $-$ $\Delta^{i+1}_-$ which is equal to $\{e3, e12, e15\}$ $-$ $\{e3, e4, e7, e10, e26\}$ $=$ $\{e12, e15\}$. Now we have all the \textit{addition-only} batches for deriving the snapshots from $\Delta^{c(c1,c2)}_+$. 
\fi


\begin{figure}[!b]
    \centering
    \includegraphics[width=1.0\columnwidth]{diagrams/schedules.pdf}
\captionsetup{justification=centering}
    \caption{Query Evaluation Schedules: (TG) Triangular Grid; ($Tree_1$, $Tree_2$) Two Trees Corresponding to Query Evaluation Schedules with Different Costs. }%\nael{Something is off in the figure (I think the 2 from Tree 2 went to a new line and overlaps with Cost in red)}
    \label{fig:treeschedules}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{diagrams/algorithm.pdf}
    \vspace{-0.2in}
    \caption{Algorithm Steps: (a) Create TG; (b) Identify Steiner Tree; and (c) Bypass nodes with indegree and outdegree of 1.} 
    \label{fig:example_work-sharing}
    %\vspace{0.025in}
\end{figure*}

\input{algo-first.tex}

\paragraph*{Query Evaluation Schedules:} Every tree rooted at $G_c$ and including all leaves (snapshots) represents a query evaluation schedule. For our example, the TG representation and two query evaluation schedules are shown in Figure~\ref{fig:treeschedules}. Recall that for this example, in the preceding section, we had shown that the cost of direct-hop schedule is 22 additions. However, when we consider the two trees shown here, their costs are 19 additions (for $Tree_1$) and 21 additions (for $Tree_2$).  
This is because both the schedules shown take advantage of additional \emph{work sharing}: in $Tree_1$, by including $ICG_1$, we can share additions that are common to $G_i$ and $G_{i+1}$ but not present in $G_{i+2}$; and in $Tree_2$, by including $ICG_2$, we can share additions that are common to $G_{i+1}$ and $G_{i+2}$ but not present in $G_i$.  In other words, the edges that are traversed multiple times are only computed once stopping at the ICG where the paths diverge, reducing the number of additions through work sharing.

While the reduction in number of total additions in the above example is small, it should be noted that this reduction will grow as the number of snapshots grows because, especially in higher levels of the TG, each edge can lead to many snapshots and would have been added independently and redundantly for each snapshot in direct-hop.  Moreover, a secondary factor is that the size of $G_c$ becomes smaller as the number of edge additions and deletions increases with more snapshots, leading to more unexploited work sharing opportunities among the subsequences of snapshots grow. %\nael{I am not sure this is the main reason.  The main point is that more snapshots have more in common and therefore benefit from work sharing even if the root GC is of similar size.  Otherwise edges near the top of the TG would be traversed many many times.} 
Finally, note that when there is a path from $G_c$ to a leaf snapshot which passes through an $ICG$ which has exactly one incoming and outgoing edge in the $Tree$ identified, we simply bypass the node and combine the addition batches for incoming and outgoing edges into one larger batch to maximize parallelism. In our example, in $Tree_1$ we bypass $ICG_2$ and in $Tree_2$ we bypass $ICG_1$. 


\iffalse
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{diagrams/picture4.pdf}
    \caption{Showing different paths from the \textit{CoreGraph} $G_c$ to the second snapshot $G_{i+1}$. There are six different paths from $G_c$ to $G_{i+1}$, and the first two paths are the most optimum and have the same cost. }
    \label{fig:different_paths}
\end{figure}
\fi



\iffalse
If you see Figure~\ref{fig:different_paths}, we have multiple paths from the \textit{CommonGraph} to our snapshots. This section will analyze different paths, from the \textit{CommonGraph} to the snapshots. For example, let us consider all the paths from $G_{c(c1,c2)}$ to $G_{i+1}$. Here are all the paths: 
\\
\\
$Path1:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c1(i,i+1)}$ $\xrightarrow[]{}$ $G_{i+1}$ \\
$Path2:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c2(i+1,i+2)}$ $\xrightarrow[]{}$ $G_{i+1}$ \\
$Path3:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c1(i,i+1)}$ $\xrightarrow[]{}$ $G_{c2(i+1,i+2)}$ $\xrightarrow[]{}$ $G_{i+1}$ \\
$Path4:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c2(i+1,i+2)}$ $\xrightarrow[]{}$ $G_{c1(i,i+1)}$ $\xrightarrow[]{}$ $G_{i+1}$ \\
$Path5:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c1(i,i+1)}$ $\xrightarrow[]{}$ $G_{i}$ $\xrightarrow[]{}$ $G_{i+1}$ \\
$Path6:$ $G_{c(c1,c2)}$ $\xrightarrow[]{}$ $G_{c2(i+1,i+2)}$ $\xrightarrow[]{}$ $G_{i+2}$ $\xrightarrow[]{}$ $G_{i+1}$\\
\\
For the $path1$, first we should to add $\{e4, e7, e10, e26\}$ to $G_{c(c1,c2)}$ to reach $G_{c1(i,i+1)}$, and then we should add a set of $\{e3, e12, e15\}$ to $G_{c1(i,i+1)}$ to get $G_{i+1}$. For the $path2$, first we need to add $\{e12, e15\}$ to $G_{c(c1,c2)}$ to get $G_{c2(i+1,i+2)}$, and then we need to add $\{e3, e4, e7, e10, e26\}$ to $G_{c2(i+1,i+2)}$ to get $G_{i+1}$. These two paths are the most optimum directions to reach $G_{i+1}$ from $G_c$. The following sections will prove that these two paths are the best directions and have the same cost. If we combine both addition batches in each direction into one addition batch, both path1 and path2 have the same addition batch, and it is equal to $\{e3, e4, e7, e10, e12, e15, e26\}$. In those two paths, we only have additions. 

In $path3$, first we should to add a set of $\{e4, e7, e10, e26\}$ to $G_{c(c1,c2)}$ to reach $G_{c1(i,i+1)}$, and then we should add a st of $\{e12,e15\}$ and delete $\{e4,e7,e10,e26\}$ to get $G_{c2(i+1,i+2)}$, finally we should add $\{e3, e4, e7, e10, e26\}$ to $G_{c2(i+1,i+2)}$ and get $G_{i+1}$. In $path3$ we have a combinations of additions and deletions and the cost of this path is clearly higher than the first two paths because we added an useless extra stage in between which contains both additions and deletions. In $path4$ we should first add $\{e12,e15\}$ to $G_{c(c1,c2)}$ to get $G_{c2(i+1,i+2)}$, and then we should do a backward direction from $G_{c2(i+1,i+2)}$ to $G_{c1(i,i+1)}$. In order to go from $G_{c2(i+1,i+2)}$ to $G_{c1(i,i+1)}$ we should delete $\{e4,e7,e10,e26\}$, and add $\{e12,e15\}$ to $G_{c2(i+1,i+2)}$, and finally, we should add $\{e3,e12,e15\}$ to $G_{c1(i,i+1)}$ to get $G_{i+1}$. This path is not addition-only because we have a backward direction on this path. The cost of this path is also higher than the cost of the first two paths because we also need to add an extra stage to this path, and also this path contains deletion, which has a higher cost compared to addition. 

In $path5$ first we should to add $\{e4, e7, e10, e26\}$ to $G_{c(c1,c2)}$ to get $G_{c1(i,i+1)}$, and then we should add $\{e9,e11,e16,e23,29\}$ to $G_{c1(i,i+1)}$ to get $G_i$, finally we should delete a set of $\{e9,e11,e16,e23,e29\}$ and add  $\{e3,e12,e15\}$ to $G_i$ to get $G_{i+1}$. In the direction we have deletions and the cost of this direction is clearly bigger than the cost of the first two directions because in this direction we added an extra stage in between which contains deletions. In $path6$ we will go from $G_{c(c1,c2)}$ to $G_{c2(i+1,i+2)}$ by adding $\{e12,e15\}$, and then we can go from $G_{c2(i+1,i+2)}$ to $G_{i+2}$, by adding $\{e9,e11,e14,e24,e29\}$, finally we can go from $G_{i+2}$ to $G_{i+1}$ by adding a set of $\{e3,e4,e7,e10,e26\}$ and deleting $\{e9,e11,e16,e23,e29\}$. This path is also contains deletions and we have an extra stage here which has higher cost compare to $path1$ and $path2$. 


Therefore, we can conclude that the common subgraph's direct paths to each snapshot are the most optimum path. To have an abstract view of the problem, we can remove the intermate common subgraphs like Figure~\ref{fig:different_paths}. As we can see in Figure~\ref{fig:different_paths}, we only have one path from \textit{CommonGraph} $G_c$ to the three snapshots $G_i$, $G_{i+1}$, and $G_{i+2}$. We should add $\Delta^{c1}_+$ to $G_c$ to get $G_i$. If you see Figure~\ref{fig:paths_combination}, $\Delta^{c1}_+$ is the result of adding $\Delta^{c(i)}_+$ and $\Delta^{c1(i)}_+$. We can derive $G_{i+1}$ from $G_{c}$ by adding $\Delta^{c2}_+$ to $G_{c}$. We can find $\Delta^{c2}_+$ by adding $\Delta^{c(c1)}_+$ to $\Delta^{c1(i+1)}_+$ or by adding $\Delta^{c(c2)}_+$ to $\Delta^{c2(i+1)}_+$. $G_{i+2}$ can be derive by adding $\Delta^{c3}_+$ to $G_c$ and as we can see in the Figure~\ref{fig:paths_combination}, $\Delta^{c3}_+$ is the result of adding $\Delta^{c(c2)}_+$ to $\Delta^{c2(i+2)}_+$. Therefore, we can combine all the intermediate addition batches in one addition batch and add it once to the core graph and get the snapshot, but this approach has a problem. As shown in Figure~\ref{fig:paths_combination}, here is the cost of finding each snapshots from core graph:\\
\\
$Cost(G_i)$ $=$ $\Delta^{c(c1)}_+$ $+$ $\Delta^{c1(i)}_+$ \\
$Cost(G_{i+1})$ $=$ $\Delta^{c(c1)}_+$ $+$ $\Delta^{c1(i+1)}_+$ \\
$Cost(G_{i+2})$ $=$ $\Delta^{c(c2)}_+$ $+$ $\Delta^{c2(i+2)}_+$ 
\\

As you can see in the above equations, for computing the $G_i$ and $G_{i+1}$, we have the common addition batch computation of $\Delta^{c(c1)}_+$. Thus, we will compute this addition batch twice for the first two snapshots.

\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{diagrams/picture5.pdf}
    \caption{Showing the best path from the common subgraph to each snapshot, the best path is the direct path without any forward or backward direction, which only contains addition.}
    \label{fig:paths_combination}
\end{figure}

\subsection{CommonGraph Based Direct-Hop Algorithm}
\label{work sharing}

As shown in Figure~\ref{fig:example_work-sharing}, we have four different snapshots of graph G at different time points ($G_i$, $G_{i+1}$, $G_{i+2}$, $G_{i+3}$). We have created the common subgraph tree, and the final common subgraph for all snapshots is $G_c$. As discussed in the previous section, the best path from $G_c$ to different snapshots is the direct path, and if we have multiple paths from the common subgraph to a snapshot, the cost of all the paths is the same. We have one direct path from $G_c$ to G1, and it passes from $G_{c4}$ and $G_{c1}$. For this path, we should add \{$\Delta^{1}_+$ $+$ $\Delta^{3}_+$ $+$ $\Delta^{7}_+$\} to $G_c$. We have thee direct paths from $G_c$ to $G_{i+1}$, and the cost of these paths is the same. The first one passes from $G_{c4}$ and $G_{c1}$. The second one passes from $G_{c4}$ and $G_{c2}$, and the third path passes from $G_{c5}$ and $G_{c2}$. The cost of all these three paths is equal, and as an instance, we pick the first path, which passes from $G_{c4}$ and $G_{c1}$.  For this path, we should add \{$\Delta^{1}_+$ $+$ $\Delta^{3}_+$ $+$ $\Delta^{8}_+$\} to $G_c$. We also have three different direct paths for deriving $G_{i+2}$ from $G_c$ with equal costs; for an instant, we pick the path which passes from $G_{c4}$ and $G_{c2}$. For this path, we should add a batch of addition \{$\Delta^{1}_+$ $+$ $\Delta^{4}_+$ $+$ $\Delta^{10}_+$\}. Therefore, we should add the following addition batches to $G_c$ for finding $G_i$, $G_{i+1}$, and $G_{i+2}$ from $G_c$: 
\\
\\
Addition batch for $G_i$ \hspace{0.27cm}$=$ \{\textcolor{red}{$\Delta^{1}_+$} $+$
\textcolor{cyan}{$\Delta^{3}_+$} $+$ $\Delta^{7}_+$\}\\
Addition batch for $G_{i+1}$ $=$ \{\textcolor{red}{$\Delta^{1}_+$} $+$ \textcolor{cyan}{$\Delta^{3}_+$} $+$ $\Delta^{8}_+$\}\\
Addition batch for $G_{i+2}$ $=$ \{\textcolor{red}{$\Delta^{1}_+$} $+$ $\Delta^{4}_+$ $+$ $\Delta^{10}_+$\}\\
\\
As shown in the above equations, we should add $\Delta^{1}_+$ to $G_c$ three times for computing three snapshots, and also, we should add $\Delta^{3}_+$ two times to $G_c$ for computing two snapshots. Therefore, we have so many common computations for getting all the snapshots, especially when we increase the number of snapshots. To solve this problem, we are proposing the work-sharing algorithm. 
\fi



\vspace{-0.075in}
\paragraph*{Complete Algorithm for Finding Minimum Cost Query Evaluation Schedule}
%Our goal in the work-sharing algorithm is to remove adding the same edges in the CommonGraph tree structure when we are traversing the tree. Let us first explore the algorithm using an example, and then we will see the algorithm's pseudocode. We only compute each addition batch once for all the snapshots in the work-sharing algorithm. In Figure~\ref{fig:example_work-sharing}, we have shown an example of the CommonGraph algorithm. 
The algorithm consists of three steps as shown in Figure~\ref{fig:example_work-sharing}. In the first step, we will create the \emph{Triangular Grid} TG for a given sequence of snapshots on which a user query needs to be evaluated. The optimal query evaluation schedule consists of the tree that reaches all the snapshots with minimum total cost; this minimum cost represents the maximal degree of reuse, allowing the cost to drop to this minimal from the direct-hop cost which has no reuse.  This problem is the Steiner tree problem~\cite{hwang-92}.  Thus, the second step of our algorithm finds the best paths from $G_c$ to all the snapshots using the Steiner tree algorithm that finds a minimum cost tree $Tree$, that is, the sum of additions labelling the edges included in $Tree$ is the minimum. Finally, in the third step, we bypass $ICG$ nodes that have exactly one incoming and one outgoing edge in $Tree$ and merge the edge addition batches for individual edges into one batch corresponding to the union of the edge batches on the incoming and outgoing edges of each bypassed ICG. In Figure~\ref{fig:example_work-sharing} we can bypass nodes and combine batches $\Delta^{1}_+$ and $\Delta^{3}_+$ into one batch and also combine $\Delta^{2}_+$ and $\Delta^{6}_+$ into one batch.

The pseudocode of the above three step process is given in Algorithm~\ref{algo:tree_construction}. It should be noted that this algorithm is general in two respects. First, it handles an \emph{arbitrary number of snapshots}, i.e. it builds the TG with appropriate number of levels. Second, since it supports bypassing, it \emph{subsumes the direct-hop solution}, i.e. it is perfectly capable of generating the direct-hop query schedule if all the available sharing can be achieved by the $G_c$ graph and no additional sharing opportunities exist among subsequences of snapshots.

%You can see the algorithm for creating the CommonGraph tree with a minimum cost in Algorithm~\ref{algo:tree_construction}. The algorithm has two inputs, the first input is our snapshots, and the second input is addition and deletion batches for our snapshots. The output of the algorithm is the minimum cost CommonGraph tree. We divide the algorithm into three parts. First, we should create the CommonGraph tree using our snapshots and out deletion and addition batches. In this part, for each $G_i$ and $G_{i+1}$ in our snapshot list, we will compute the weight of the edge to the left child ($w_1$) and the weight of the edge to the right child ($w_2$) of each node in the tree. After construction of the CommonGraph tree, we should prune that to find the minimum cost paths from $G_c$ to all the snapshots. Therefore, we will use the Steiner algorithm for the step. Based on the Steiner algorithm, we will make the $G_c$ and all the snapshots as terminals, and then we will start to compute the best paths. In the last step of the algorithm, we will combine the edges of the vertices where they only have one incoming edge and one outgoing edge. 



==> background.tex <==
\section{Limitations of Existing Systems and \\ Overview of CommonGraph}\label{background}


% Tegra: 
% 1. a brief background on graph-parallel systems 
% 2. describe various types of time-evolving graph workloads
% 3. The limitations of existing systems are discussed
% 4. before we layout the challenges in enabling efficient ad-hoc analytics on evolving graphs

% Our Paper:
% 1. a brief background on streaming graph systems and streaming system
% 1.2. state of art and limitation?
% 1.3 analysis of performance with streaming-graph system
% 1.4. kickstarter introduction and limitation
% 2. evolving graph benchmark
% 5. Motivation
In this section, we discuss the factors that limit the performance of existing evolving graph processing systems and then provide an overview of \emph{CommonGraph} and how it overcomes these limitations.

\begin{figure}[!t]
    \vspace{-0.1in}
    \centering
    \includegraphics[width=0.99\columnwidth]{diagrams/computation.pdf}
    \includegraphics[width=0.85\columnwidth]{diagrams/mutation.pdf}
  \captionsetup{justification=centering}
    \caption{Kickstarter~\cite{kickstarter} Costs: (Top) Computation Cost of Deletions vs. Additions; and (Bottom) Graph Mutation Cost.}
    \label{fig:motivate}
    \vspace{-0.15in}
\end{figure}

\subsection{Dynamic Graph Workloads and Systems}
Dynamic graph systems can be categorized into streaming graph and evolving graph systems. A streaming graph system maintains a single version of the changing graph and, using incremental algorithms, continuously updates the results of a query as the graph is modified to maintain the query solution relative to the latest graph.  To amortize the cost of streaming, typically updates are batched. An evolving system evaluates a query on multiple snapshots of a graph, that can stretch over a large time window, extracting historical/trend data. It may carry out query evaluation on multiple snapshots in parallel or start with one snapshot at a time and leverage incremental algorithms developed for streaming systems to reach others.

Let $G_t$ represent the snapshot of a dynamic graph at snapshot $t$. At snapshot $t+1$, the graph changes to $G_{t+1}$ via application of two \emph{batches of updates}, a batch of edge additions $\Delta^{t}_+$ and a batch of edge deletions $\Delta^{t}_-$. In a streaming graph system a single version of graph is maintained, i.e. $G_t$ changes to $G_{t+1}$ after application of batches of updates (i.e., $\Delta^{t}_+$ and $\Delta^{t}_-$). In an evolving graph scenario multiple snapshots of the graph [$G_{t_0}$, $G_{t_1}$, $G_{t_2}$, ..... $G_{t_n}$] are considered (e.g., for a transportation network, the snapshots may correspond to different amounts of traffic at different times of the day, or across different days of the week). If the snapshots are very far away from each other in time, streaming a large batch of updates may be more expensive than evaluating the query on the two snapshots independently. However, if snapshots are closer in time (more accurately, the number of updates is not excessive), then the incremental algorithms used by streaming systems can be leveraged to avoid redundant recomputation.

When incremental algorithms are being leveraged, after evaluating the query on one snapshot, the graph for the snapshot is first mutated (i.e., the data structures are changed in place) to obtain the one for the other snapshot and then the incremental algorithm is used to update query results. A primary observation that motivates \emph{CommonGraph} is that when the system has to handle both deletions and additions, the cost of incremental computation that handles deletions is significantly higher than that for additions. Moreover, the cost of graph mutations is also significant. In Figure~\ref{fig:motivate} these effects are shown for the Kickstarter~\cite{kickstarter} system. The incremental cost of processing a batch of deletions is nearly 3$\times$ the cost of processing an equal number of additions, and this observation holds across batches of different sizes. Handling deletions is more expensive because the algorithm is more complex for monotonic algorithms and impacts on query results are more widespread across the graph, necessitating significantly more processing. Finally, Kickstarter's cost of graph mutation is also several times greater for deletions than additions.

%To understand the limitation within the existing system, we do profiling with Kickstarter, one of the state of art streaming graph system, we identify the addition and deletion query with different number of batches, the figure shows that with the batch size increase, the time for deletion computation increase greatly over the time consumption with insertion computation, which will heavily affect the computation for snapshots differs from the original graph greatly.

%RELATED WORK. Previous works (e.g., Kineograph, Differential-Dataflow, Kickstarter, GraphBolt) are focused on providing accurate incremental algorithm but lack of ability to process arbitrary snap-shots with time-evolving graph workloads (ad-hoc operation in Tegra). Also, none of the existing streaming system supports multiple snapshots storage. Some evolving-graph system (e,g., Chronos~\cite{chronos}, Immortal-Graph, GraphOne~\cite{graphone}, Tegra~\cite{tegra}) focus on providing efficient storage for multiple snapshots and concurrent querying but lack of ability to perform incremental computation, while the others (e.g., LLAMA,) use multi-version array to support incremental computation but suffer from low efficiency for new graph mutation. One of the state of art system named Tegra supports both incremental operation, however the persistent adaptive radix tree (pART) structure brings overhead for push operation than streaming system, makes it slower in pure incremental operations. 

%To understand the performance overhead for multi-version control in existing evolving-graph system, we pick Aspen as a baseline, we run single snapshots query on Aspen and ligra system. Figure shows the percentage of overhead for different algorithm runs on ligra and Aspen with different graph. Apart from the storage overhead, none of the evolving graph system can fully support the work-sharing query over different snapshots, but the working-sharing scenario happens quite often in our daily life. For example, in social network, John and Emily followed and unfollowed each other several times, their connections will be recomputed unnecessary multiple-times in real-life graph system. To reveal the potential redundancy reduction opportunity, we developed delicate algorithm illustrated in section. 

%Summing up the limitations from current dynamic graph systems, we can clarify the challenges for designing the evolving-graph system in two perspectives: 1.flexible graph mutation and snapshot construction ; 2. fast and efficiently incremental graph query. To resolve the challenges, we proposed a tree-structure which starts from a root graph commonly shared across time series, and we also improve the incremental algorithm from current state-of-art streaming graph system to suits our needs.



% \subsection{State of Art system and Limitations}
% \vspace{0.2in}
% In this section, we discuss the limitation in the existing dynamic-graph systems, which can be categorized as stream-graph system and evolving-graph system.
% \vspace{0.2in}

%\subsection{Static Graph Systems}
%Popular used graph processing model is the vertex-centric programming model, which first developed based on bulk synchronous parallel (BSP) model by Pregel. Initial from the default initial vertex values, the pre-defined vertex function which varies from different algorithms are applied across all vertices (or part) of the graph, the computation process continue iteration by iteration after the vertex values become stable. 
%Other model have been proposed too, such as edge-centric model that takes streaming edge lists as input, subgraph-centric model which requires pre-procssing input graph for redundancy reduction, and path-centric model which benefits  monotonic algorithms by providing path-level parallelism. The design of the dynamic graph system naturally mathes the vertex-centric paradigm, consider the situation when a new edges are inserted to the graph, the reevaluation starts directly from the converged vertex of previous iteration, instead of re-initialize from the begining of the computation. For correctness insurance, the source vertex of the inserted edge needs to be schedule to the frontier, which restart the query until the whole graph becomes stable once again, in this incremental query, the push operation from vertex-centric model can't be replaced by pull operation from edge-centric paradigm and the heavy pre-processing from sub-graph or path-centric becomes huge burden.
%\subsection{Dynamic Graph Systems}


\subsection{CommonGraph: Converting Deletions to Additions}

To address the above problems (i.e., the high incremental cost of deletions and the significant cost of mutation), our system shown in Figure~\ref{fig:overview} based on \emph{CommonGraph} introduces these three complementary techniques. The graph is represented in form of the shared \emph{CommonGraph} and additional batches of edges ($\Delta$ batches) that can be used in conjunction with the \emph{CommonGraph} to realize different snapshots. This representation of the graph and its updates allows different query evaluation schedules (shown as red arrows) to be realized that do not require deletions, incorporate work sharing, and do not require explicit graph mutation. Next, we provide an overview of these three features.

\begin{figure}[!h]
    %\vspace{-0.125in}
    \centering
    \includegraphics[width=1.0\columnwidth]{diagrams/overview.pdf}
    \caption{Our Approach.}
    \label{fig:overview}
        %\vspace{-0.125in}
\end{figure}

\paragraph*{Converting Deletions to Additions} To overcome the high computational cost of processing edge deletions, we make a key observation: all deletions can be converted to additions by computing a \emph{CommonGraph} that includes only the edges that are common to all the snapshots under consideration. Once query results have been computed on this graph, then results for any snapshot can be computed by \emph{adding the batch of missing edges} to the \emph{CommonGraph} and employing the incremental algorithm to update query results. That is, we can avoid the use of the more expensive incremental algorithm for deletions since deletions become additions if we reverse the order in which the snapshots are processed. %Note that the use of \emph{CommonGraph} naturally leads to \emph{work sharing} across the computation for the two snapshots.

Figure~\ref{fig:common_graph_example} illustrates how \emph{CommonGraph} converts deletions into additions. The top two graphs represent two snapshots of the evolving graph. The standard streaming approach will apply $\Delta^{i}_+$ edge additions and $\Delta^{i}_-$ deletions to update query results for the first snapshot $G_i$ and obtain the query results for second snapshot $G_{i+1}$. On the other hand, by creating the \emph{CommonGraph} $G_c$, we can incrementally update query results for $G_c$ via independently performing edge additions $\Delta^{i}_+$ and $\Delta^{i}_-$ to obtain results for $G_i$ and $G_{i+1}$.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\columnwidth]{diagrams/picture2.pdf}
\captionsetup{justification=centering}
    \caption{\textit{CommonGraph} $G_c$ for two snapshots $G_i$ and $G_{i+1}$; the latter is created via a  $\Delta^{i}_+$ additions (blue edges) and $\Delta^{i}_-$ deletions (red edges); going from $G_c$ to $G_i$ and $G_{i+1}$ requires only addition of $\Delta^{i}_-$ and $\Delta^{i}_+$ respectively.}
    \label{fig:common_graph_example}
    \vspace{-0.15in}
\end{figure}

\paragraph*{Work Sharing for a Large Number of Snapshots}
Although the \emph{CommonGraph} achieves work sharing among all the snapshots to process the common graph itself, as the time window grows and the number of snapshots increases, additional opportunities for work sharing of the graph updates among subsets of snapshots arise.  Specifically, any subset of the snapshots may share additional edges in common (for example, if we constructed the common graph just for that subset), and can share work if we stream the additional edges to reach this larger common graph together instead of each query adding them separately to each snapshot.  Let us assume that we have $n$ snapshots to consider. Our second contribution, the \emph{Triangular Grid} (TG) representation, allows systematic exploration and discovery of a $n$ incremental computations that result in query results for all $n$ snapshots while at the same time maximizing the overall \emph{work sharing} beyond the base level of sharing that the \emph{CommonGraph} naturally achieves. 

The TG representation incorporates original snapshots, the \emph{CommonGraph} representation, and many intermediate \emph{CommonGraph}s that correspond to \emph{CommonGraphs} for subsequences of original snapshots. Edges connecting snapshots are labeled with batches of edge additions that convert one \emph{CommonGraph} into another representing a smaller sequence of snapshots. We show that solving the Steiner Tree problem on the \emph{Triangular Grid} representation identifies the sequence of transitions through the grid that maximizes reuse.  Algorithms for constructing the TG representation and finding the set of incremental computations that maximize work sharing are discussed in the next section.

%Apart from avoiding complex deletion operation and expensive graph mutation operation, tree-based storage structure also provides us the opportunity for work sharing across different snapshots. For example, in the figure a web network needs to be queried three times to report network traffic situation in 8:00 am, 16:00 pm and 17:00 pm. Obviously three graph queries on three different snapshots are expensive and inefficiently, however, with the tree-based management, we can start from the pre-compute root graph, which also represent the static part during the whole day, and we can simultaneously processing three independent incremental query, moreover, since second and third snapshots are quite similar, we only need to pay the computation overhead for small incremental queries.   

\paragraph*{Evolving Graph Representation for Evaluating Query.} Besides the two algorithmic contributions above, we also identify a significant source of overhead in streaming graph systems. Specifically, we observe that there is a high cost of mutation --updating the graph representation -- for converting one snapshot into another.  To address this overhead, we introduce a new representation that significantly reduces the mutation overhead. In addition to the Compressed Sparse Row (CSR) representation of the \emph{CommonGraph}, we also create CSR representations of the batches of edges that correspond to edges that transition from one node to another in the TG. This way, the \emph{CommonGraph} is never changed but rather batches of additional edges that need to be added to the \emph{CommonGraph} to obtain an intermediate or final snapshot are simply loaded to augment the \emph{CommonGraph}.  Different snapshots are thus represented by the set of additional edges they include.
%used in conjunction with the \emph{CommonGraph}.

Next we present 
the \emph{Triangular Grid} representation and algorithms for finding query evaluation schedule to exploit \emph{work sharing}.

%Incremental computation clearly reduces the number of computation required in dynamic graph system, however, deletion operations are much expensive then addition operations since deletion operation often involves back propagate operation to retrieve the information in the previous time slot.
%To avoid the birth defects in incremental algorithm, we provides tree-based graph representation which consists a common graph from multiple snapshots and piles of edges arrays transformed from insertion/deletion batches between different snapshots, more detailed illustrated in section. Figure illustrated a example when we query a new snapshot, the push operations from the active vertex will perform on both common graph and all the small edge arrays that constructed the snapshot.



% \vspace{0.1in}
% Scenario like "how many friends Andrew have in year 2018, 2019 and 2020?", requires multi-queries with different snapshots, to resolve these consideration, we develop parallel execution paradigm, to which users only need to provide the snapshots' number and query algorithm for computation. 
% Apart from this, dynamic evolving graphs typically have small difference over different snapshots, previous systems like capture this features and created common graph among them and applied incremental algorithm to avoid the repeated queries over them same part of the graph. However, the smallest graph over hundreds of snapshots can be pretty small with many disconnected components, which leads to less computation sharing. Nevertheless, graph mutation can also take great amount of time in those systems, which can be big burden to tradition sparse data structure utilized in them. In our system, we proposed tree-based graph snapshots organization which supports concurrently execution without expensive graph mutation. Also, we introduce path finding algorithm which maximize the sharing workloads in parallel queries execution. The path finding algorithm can also be seen as a learning algorithm, one query in the tree-based snapshots system will be the learning object for other snapshots evolved from it, multiple concurrent queries can be represented as multiple learning paths, which construct the self-learning dynamic graph system.
% \vspace{0.1in}
% \subsubsection{workloads sharing over different snapshots}
% \vspace{0.1in}
% New graph snapshots construction is often considered as offline algorithm compare to graph queries computation, in our system, we provide tree structure illustrated in section, to support new snapshots construction. We take edge addition and deletion as input and based on the previous snapshots, the memory-friendly new constructions will be push into the system.

% Based on the challenges, we proposed our 

% \vspace{0.2in}

% \subsubsection{flexible limitation}
% \vspace{0.2in}
% Table compares the different features supported by existing streaming and evolving graph system compared to our proposed system. Streaming systems are normally lack of ability to support flexible access to different graph snapshot in different time-stamp, and evolving graph systems suffer from frequently queue whole graph whenever we want to process a new snapshot from the system.
% \subsubsection{Algorithm limitation}
% \vspace{0.2in}
% Figures compares the different execution time for addition and deletion for graph mutation and incremental algorithm in different system, we can make an observation that addition requires much less execution time in both graph mutation and incremental algorithm, considering this, we present an algorithm to eliminate all deletion in evolving graph system, more details can be seen in section.
% \subsubsection{Concurrency limitation}
% \vspace{0.2in}
% From Table, we can see that none of the existing systems supports queuing multiple snapshots concurrently in the system, to supports concurrently execution, we developed the algorithm which can queue multiple graph in the same time, more details can be seen in section.

%\vspace{-1mm}




==> conclusion.tex <==
\section{Concluding Remarks}

Graph analytics on a dynamic graph that evolves over large time scales is a challenging problem.  A user is typically interested in queries that span potentially large time windows, which translates into having to solve sub-queries targeting snapshots of the graph within those windows.  We propose new algorithms that significantly improve the performance of evolving graphs compared to state-of-the-art streaming graph systems.  In particular, we observe that deletions are significantly more expensive than additions, and that streaming from one original snapshot limits opportunities for work sharing.  We propose \emph{CommonGraph}, a representation of an evolving graph that captures the part of the graph that is common among a group of snapshots.  Moving from this graph to any snapshots can be accomplished by adding the missing edges needed for the particular snapshot.   We also show that \emph{CommonGraph} exposes opportunities for work sharing among snapshots that share groups of edges, and capitalize on this opportunity using a Triangular Grid structure, that enables optimal work sharing when computing queries across a sequence of snapshots.  Finally, we observe that streaming implementations incur substantial cost to mutate the graph as it changes, and come up with a representation that enables composing representations in place to represent the different snapshots without mutation.  Taken together, our ideas result in 1.38$\times$ to 8.17$\times$ improvement in the evaluation of five query types, an advantage that grows with the number of snapshots being analyzed.

%Nael: can omit the next paragraph 
We believe that \emph{CommonGraph} offers additional opportunities and advantages.  It breaks the sequential dependency in streaming algorithms since we are able to move to each snapshot independently of the prior ones.  This offers opportunities for parallel execution to further improve performance.  It also enables efficiencies in storage and query execution: for example, it enables efficient range queries without having to start from an initial stored snapshot that can be far from the start of the range, and therefore requires substantial overhead just to reach the first snapshot.   We intend to pursue these ideas in future work

%This paper design to efficiently handle hundreds of snapshots evolving graph computation. The key contribution in lies in three perspective, 1. addition-only and none-mutation incremental algorithm which supports streaming applications in evolving graph workloads; 2. tree-based snapshots-organization structure, which supports concurrent queries over multiple graph; 3. path-selection learning algorithm which takes advantage of tree organization to provide reduction for repeated computation. Experiments showed that our system achieves speedup over state-of-art streaming graph system, and compared to multi-snapshots evolving systems, we achieves speedup and memory efficiency over memory footprints. Besides, our concurrent results further improve performance by over current dynamic graph systems. In the future, we will explore the possibility of utilizing the system concurrency to support multiple batch queries with different sources in other dynamic graph applications.

\begin{acks}
We thank all the reviewers for their valuable feedback. This work is supported in part by National Science Foundation Grants CNS-1955650, CNS-2053383, CCF-2028714, CCF-2002554 and CCF-2226448 to the University of California, Riverside. 
\end{acks}

==> evaluation.tex <==

\section{Performance Evaluation}
All experiments are conducted on a shared memory system, which contains 56 Intel Xeon E5-2680 processor and 520GB memory. The \textbf{CommonGraph} system is compiled by g++ 7.3.1 and runs on CentOS Linux 7.

We evaluate \emph{CommonGraph} on five benchmarks (all monotonic algorithms).  The benchmarks are shown in Table~\ref{opt}, along with their push operations, which is the primary difference between the benchmarks.   We use the four input graphs shown in Table~\ref{graphs}. Update batches consisting of edge additions and deletions are generated for each benchmark to transition from one snapshot to the next, and the evaluation targets a number of snapshots specified with each experiment.  %In Table~\ref{opt}, we can see the different algorithms we used for the evaluation with their push operations. 

\begin{table}[ht]
\captionsetup{justification=centering}
\caption{Edges and Vertices of the Input Graphs.}
\label{graphs}
\vspace{-0.1in}
%\small
\centering
{\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|c|c|c|} \hline
Input Graph & | Edges | &\!\!| Vertices |\!\! & \!\!|Avg degree|\!\!\\ \hline \hline
LiveJournal (LJ)~\cite{LJ_backstrom} & 70M & 4M & 28.26\\ \hline
% Orkut (OR)~\cite{mislove2007measurement} & 120M & 3M & 40\\ \hline
DBpediaLinks (DL)~\cite{10.1007/978-3-540-76298-0_52} & 170M & 18M & 18.85\\ \hline
WikipediaLinks (Wen)~\cite{wikipedia}\!\!& 400M & 13M & 64.32\\ \hline
Twitter (TTW)~\cite{ttw} & 1.5B & 41M & 70.51\\ \hline
\end{tabular}
}
\end{table}

\begin{table}[!t]
\captionsetup{justification=centering}
\caption{Benchmarks and their Push Operations. CASMIN(a; b) sets a = b if b < a atomically; CASMAX is similarly defined. The algorithms are Breadth First Search (BFS), Single Source Widest Path (SSWP), Single Source Narrowest Path (SSNP), Single Source Shortest Path (SSSP), and Virterbi.}
\label{opt}
\vspace{-0.05in}
%\small
\centering
\begin{tabular}{|l|l|} \hline
Algorithm
%& \textsc{Needed} $( e(u,v) )$ \\ 
& EdgeFunction $( e(u,v) )$ \\ \hline \hline

BFS
%& $Val(v) < min( Val(u)+1, val(v))$ \\
& $CASMIN( Val(v), min( Val(u)+1, val(v) ) )$ \\ \hline

SSWP
%& $Val(v) < min( Val(u), wt(u,v) )$ \\
& $CASMAX( Val(v),  min( Val(u), wt(u,v) ) )$ \\ \hline

SSNP
%& $Val(v) > max( Val(u), wt(u,v) )$ \\
& $CASMIN( Val(v),  max( Val(u), wt(u,v) ) )$ \\ \hline

SSSP
%& $Val(v) > Val(u) + wt(u,v)$ \\
& $CASMIN( Val(v),  Val(u) + wt(u,v) )$ \\ \hline

Viterbi
%& $Val(v) < Val(u)/wt(u,v)$ \\
& $CASMAX( Val(v),  Val(u) / wt(u,v) )$ \\ \hline

\end{tabular}
\vspace{-0.175in}
\end{table}

Our first experiment tracks the execution time for evaluating a query of each of the five benchmarks on 50 consecutive snapshots. Each snapshot is separated from the next by a batch of 75,000 edge changes split \emph{evenly} between additions and deletions, which represents approximately 0.01\% of the number of edges in LiveJournal, the smallest benchmark among our input graphs. The first row for each benchmark in the table is baseline \emph{KickStarter}: we start from the initial snapshot and stream in the batches to reach the next snapshot repeatedly until we reach the final snapshot.  The second row for each benchmark uses \emph{CommonGraph} but \emph{Direct-Hop}s the additions to reach each snapshot in a single batch; although the snapshots can be processed in parallel, we report the total sequential time. %In this approach, we created the Triangular Grid, and then traverse it for each snapshot streaming all the additions in one batch. %The execution time in this approach is bigger compared to baseline because we are traversing the golden tree One-Hop by One-Hop. The third row belongs to the Addition-Only using the Direct-Hop approach. In this approach, like the previous approach, we are building the golden tree and AtoD graph, but we go from the AtoD graph to each snapshot directly. 
Finally, the last row introduces the maximal \emph{Work-Sharing} algorithm based upon building the TG and solving the Steiner tree to identify the paths that minimize the overall work to be able to reach all the snapshots.  Snapshots that share subsets of their path, share the processing to reach the node of the Triangular grid where they diverge; we are computing each addition batch once for the snapshots that share it. 

\begin{table*}[!t]
%\vspace{-0.1in}
%\small
\captionsetup{justification=centering}
\caption{Average Execution Times in Seconds for KickStarter with Both Additions and Deletions, and the speedup of CommonGraph Direct Hop and CommonGraph Work-Sharing Algorithm over KickStarter for 50 Snapshots.}
\label{tab:time}
\centering
\vspace{-0.1in}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l||c|c|c|c|c|} \hline
\multicolumn{1}{|c|}{\textbf{\textsf{Graph}}} & \textbf{\textsf{Query Evaluation Algorithm}} & \textsf{\textbf{BFS}} & \textsf{\textbf{SSSP}} & \textsf{\textbf{SSWP}} & \textsf{\textbf{SSNP}} 
& \textsf{\textbf{Viterbi}} 
\\ \hline \hline

\multirow{3}{*}{\textsf{\textbf{LJ}}} &
    \textsc{KickStarter Time} & 3.43s & 3.88s & 3.69s & 3.75s & 5.17s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Direct-Hop Speedup} & 1.58$\times$ & 1.07$\times$ & 1.23$\times$ & 1.18$\times$ & 1.02$\times$\\ \cline{2-7}
    & \textsc{Work-Sharing Speedup} & 1.86$\times$ & 1.43$\times$ & 1.38$\times$ & 1.43$\times$ 
    &  1.62$\times$ 
    \\ \hline \hline
\multirow{3}{*}{\textsf{\textbf{DL}}} &
    \textsc{KickStarter Time} & 27.22s & 27.64s & 27.91s & 27.51s & 31.87s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Direct-Hop Speedup} & 7.09$\times$ & 7.45$\times$ & 7.3$\times$ & 6.7$\times$ & 7.91$\times$\\ \cline{2-7}
    & \textsc{Work-Sharing Speedup} & 7.17$\times$ & 8.17$\times$ & 7.64$\times$ & 7.21$\times$ & 8.17$\times$ \\
    \hline \hline
\multirow{3}{*}{\textsf{\textbf{Wen}}} &
    \textsc{KickStarter Time} & 4.65s & 4.59s & 4.72s & 4.20s & 2.03s \\ \cline{2-7} \cline{2-7} 
    & \textsc{Direct-Hop Speedup} & 4.53$\times$ & 1.32$\times$ & 2.73$\times$ & 2.08$\times$ & 3.24$\times$\\ \cline{2-7}
    & \textsc{Work-Sharing Speedup} & 4.68$\times$ & 2.42$\times$ & 3.31$\times$ & 2.40$\times$ & 3.8$\times$\\
    \hline \hline
\multirow{3}{*}{\textsf{\textbf{TTW}}} &
    \textsc{KickStarter Time} & 10.91s & 11.73s & 11.32s & 11.31s & 15.30s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Direct-Hop Speedup} & 3.09$\times$ & 2.36$\times$ & 2.52$\times$ & 1.85$\times$ & 2.85$\times$\\ \cline{2-7}
    & \textsc{Work-Sharing Speedup} & 3.35$\times$ & 2.94$\times$ & 3.14$\times$ & 2.62$\times$ & 3.42$\times$ \\
    \hline 
% \multirow{3}{*}{\textsf{\textbf{OG}}} &
%     \textsc{KickStarter Time} &  20.31s & 20.59s & 20.43s & 21.62s & 23.46s\\ \cline{2-7} \cline{2-7} 
%     & \textsc{Direct-Hop Speedup} & 7.94$\times$ & 8.35$\times$ & 8.07$\times$ & 8.02$\times$ & 9.14$\times$\\ \cline{2-7}
%     & \textsc{Work-Sharing Speedup} & 8.28$\times$ & 9.68$\times$ & 8.46$\times$ & 9.17$\times$ & 9.2$\times$ \\
%     \hline
\end{tabular}
}
\end{table*}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{diagrams/scalibility1.pdf}
    \vspace{-0.175in}
    \caption{Execution time for KickStarter, CommonGraph Direct-Hop, and Work-Sharing.}%\nael{Jump for TTW-BFS direct-hop from 45 to 50 snapshots is suspicious.  Its the basis for our best case performance; can you please double check?}{Mahbod: I double checked that Professor Nael, there was a mistake and I fixed it.}
    \label{fig:scalibility1}
    \vspace{-0.1in}
\end{figure*}

In Table~\ref{tab:time}, we can see the speedup for \emph{CommonGraph}  with Direct-Hop (direct traversal to each snapshot); it outperforms the baseline KickStarter 1.02$\times$-7.91$\times$; even though it processes a higher number of edges compared to KickStarter, all these edges are additions and benefit also from parallelism among additions since they are processed in a single batch.  Moreover, some of the benefits come from avoiding the cost of graph mutation through our graph representation.  Additional speedup is achieved using work sharing, for an overall speedup of 1.38x-8.17x over baseline KickStarter. % We note that these numbers do not reflect additional possible efficiencies from processing the snapshots in parallel, which is not possible with KickStarter because of the sequential dependency between the snapshots.%\nael{We probably need to rephrase this if we show the parallelism potential results.}


%Figure~\ref{fig:snapshots} shows the execution time in seconds for \emph{CommonGraph} with direct hop compared to work sharing for a different number of snapshots. When the number of snapshots increases, the advantage of work sharing increases, as additional opportunities to share work among the increasing number of snapshots result in savings in execution time.
%better execution time than the Addition-Only (Direct-Hop) because when we increase the number of the snapshots, the chance for work-sharing will be increased.  

%\subsection{Scalability Analysis}

The next set of experiments evaluate the scalability of the direct hop and work sharing algorithms with respect to two different scaling parameters, number of snapshots and the batch size. We used our biggest graph (TTW) and four benchmarks (BFS, SSSP, SSWP, and SSNP) for the scalability experiment. In the first experiment we fix the batch size to 75K graph updates%\nael{Why did it change?} \textcolor{red}{Mahbod: fixed} 
and varied the number of snapshots from 5 to 50. 
%We compare the execution time for Kickstarter, direct hop, and the work-sharing algorithms. 
As we can see from Figure~\ref{fig:scalibility1}, the execution time of \emph{CommonGraph} based algorithms is superior to that of Kickstarter; the execution time for all three algorithms increases linearly with the number of snapshots. 

We also observe that for fewer snapshots the direct-hop algorithm works better than  work-sharing.  At a smaller number of snapshots, the degree of work sharing is small as each batch is reused by at most 2 snapshots.  At the same time, having to stabilize the solution at an intermediate common graph reduces the amount of parallelism available in executing a larger number of updates concurrently.  However, work sharing significantly outperforms direct hop when we increase the number of snapshots beyond 23 to 35 for different benchmarks.  %When we have fewer snapshots, we have a smaller TG, which means we do not have much to share in our TG, but when we gradually increase the number of snapshots, we have a bigger TG, and it increases the sharing when we are trying to go from the root to the snapshots. 

%\nael{Could we study the reuse degree as the number of snapshots increases?  Since we are not actually executing, we can show this for a much larger number of snapshots.} 

%\nael{I think it would also be cool to show the TG/routing tree for a large configuration to be able to make the point about the reuse degree.}

In Figure~\ref{fig:scalibility2}, we show the second analysis for the scalability. In this analysis, we fix the total number of graph updates and vary the batch size -- smaller batch size corresponds to more snapshots and more accurate picture of changes in query results. 
%We present the execution times of Kickstarter, direct-hop, and work-sharing algorithms on the TTW graph for four different benchmarks. 
As shown in the Figure~\ref{fig:scalibility2}, we start with 75K batch sizes for 50 snapshots and then increase the batch size to 375K for 10 snapshots. For the bigger batch size, the direct-hop algorithm works better compared to the work-sharing, and for the smaller number of the batch size, the work-sharing works better. This is because for smaller batch size we have a greater number of snapshots and the benefit of TG grows due to increased opportunities for sharing. 

%\nael{I think this result probably says that there is an optimal hybrid execution where you work share when the sharing degree is high and direct hop when it is low.  So, you might work share high in the TG, but direct hop after that.}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{diagrams/batch-size.pdf}
    \vspace{-0.15in}
    \caption{Execution times while batch size is varied, total number of graph updates is fixed.}
    \label{fig:scalibility2}
    \vspace{-0.05in}
\end{figure*}

\begin{table*}[ht]
\captionsetup{justification=centering}
\caption{Execution times (seconds) and speedups of parallel implementation of the Direct-Hop algorithm over KicKStarter.}
\label{parallel}
\vspace{-0.05in}
%\small
\centering
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l||c|c|c|c|c|} \hline
\multicolumn{1}{|c|}{\textbf{\textsf{G}}} & \textbf{\textsf{Direct-Hop}} & \textsf{\textbf{BFS}} & \textsf{\textbf{SSSP}} & \textsf{\textbf{SSWP}} & \textsf{\textbf{SSNP}} 
& \textsf{\textbf{Viterbi}} 
\\ \hline \hline

\multirow{2}{*}{\textsf{\textbf{LJ}}} &
    \textsc{Time} & 0.044s & 0.072s & 0.06s & 0.063s & 0.101s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Speedup} & 78.76$\times$ & 53.73$\times$ & 61.56$\times$ & 59.25$\times$ 
    & 51.14$\times$ \\ \hline \hline
\multirow{2}{*}{\textsf{\textbf{DL}}} &
    \textsc{Time} & 0.077s & 0.074s & 0.076s & 0.082s & 0.08s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Speedup} & 354.93$\times$ & 372.52$\times$ & 365.37$\times$ & 335.19$\times$ 
    & 395.64$\times$ \\ \hline \hline
\multirow{2}{*}{\textsf{\textbf{Wen}}} &
    \textsc{Time} & 0.021s & 0.07s & 0.034s & 0.04s & 0.041\\ \cline{2-7} \cline{2-7} 
    & \textsc{Speedup} & 226.17$\times$ & 66.06$\times$ & 136.89$\times$ & 104.12$\times$ 
    & 161.85$\times$ \\ \hline \hline
\multirow{2}{*}{\textsf{\textbf{TTW}}} &
    \textsc{Time} & 0.071s & 0.099s & 0.09s & 0.122s & 0.107s\\ \cline{2-7} \cline{2-7} 
    & \textsc{Speedup} & 154.54$\times$ & 118.09$\times$ & 126.11$\times$ & 92.5$\times$ 
    &  142.39$\times$ \\ \hline 
% \multirow{2}{*}{\textsf{\textbf{OG}}} &
%     \textsc{Time} & 0.051s & 0.05s & 0.051s & 0.054s & 0.051s\\ \cline{2-7} \cline{2-7} 
%     & \textsc{Speedup} & 397.22$\times$ & 414.02$\times$ & 403.91$\times$ & 401.32$\times$ 
%     &  457.10$\times$ \\ \hline 
\end{tabular}
}
\vspace{-0.1in}
\end{table*}

% We measured the overhead of our approach by testing the execution time of only addition batches in KickStarter and our evolving system. For this experiment, we used the four graphs with five benchmarks with 50 different addition batches from 35K to 1750K. Figure~\ref{fig:overhead} shows the average overhead for our four graphs and five different benchmarks. The average overhead of our approach is 1.17$\times$, which is less than the average overhead of existing evolving graph systems. This overhead is only for incremental computation for addition batches in the CommonGraph algorithm over the KickStarter. This overhead comes from the data structure because the CommonGraph algorithm holds the CommonGraph, which is the root of our TG and multiple CSR for addition batches, but KickStarter only contains one version of the graph. %In contrast, the overhead of Aspen~\cite{aspen} is 1.44$\times$ over Ligra+. 

We also varied the ratio of additions and deletions to show that across different ratios our common graph representation provides gains over KickStarter. In Figure~\ref{fig:ratio} we show the speedups by varying batches from from 150K additions and 50K deletions to 50K additions and 150K deletions. As we can see, as greater percentage of deletion updates are considered, the speedup of Direct-Hop over KickStarter increases.


%\begin{table}[!b]
%\vspace{-0.15in}
%\captionsetup{justification=centering}
%\caption{The startup execution time for KickStarter vs. CommonGraph for 50 batches 
%from 75K to 3750K 
%on the LiveJournal graph.}
%\label{overhead}
%\vspace{-0.025in}
%\small
%\centering
%{\renewcommand{\arraystretch}{1.2}
%\begin{tabular}{|l||c|c|c|} \hline
%\multicolumn{1}{|c||}{\textbf{\textsf{G}} }
% & \textsf{\textbf{KickStarter}} & \textsf{\textbf{CommonGraph}} &\!\!\textsf{\textbf{Overhead}}  \\ 
%\hline \hline
%\multirow{1}{*}{\textsf{\textbf{BFS}}} 
%& 0.024s & 0.027s & 1.17$\times$ \\ \hline 
%\multirow{1}{*}{\textsf{\textbf{SSSP}}}  
%& 0.04s & 0.046s & 1.15$\times$ \\ \hline 
%\multirow{1}{*}{\textsf{\textbf{SSWP}}}
%& 0.041s & 0.048s & 1.18$\times$ \\ \hline 
%\multirow{1}{*}{\textsf{\textbf{SSNP}}} 
%& 0.039s & 0.045s & 1.16$\times$ \\ \hline 
%\end{tabular}
%}
%\end{table}

%\nael{Any plans to show the estimated parallel execution time as the longest time to reach any snapshot?}
%\textcolor{red}{Mahbod: I added a table for this.}


\begin{figure*}[!h]
\begin{minipage}{3.25in}
    \centering
    \includegraphics[width=0.99\columnwidth]{diagrams/ratio1.pdf}
\captionsetup{justification=centering}
    \caption{Sensitivity of performance to the ratio of additions and deletions.}
    \label{fig:ratio}
%\end{figure}
\end{minipage}
%\begin{figure}[!b]
\begin{minipage}{3.25in}
   \centering
    \includegraphics[width=0.9\columnwidth]{diagrams/breakdown.pdf}
\captionsetup{justification=centering}
    \caption{Breakdown of the execution time for TTW graph for the baseline KickStarter (KS) and CommonGraph (CG) Work-Sharing algorithm.}
    \label{fig:breakdown}
\end{minipage}
\end{figure*}

\emph{CommonGraph} also exposes opportunities for parallelism that are difficult to realize in streaming only systems such as Kickstarter.  Specifically, we can execute the direct hop algorithm in parallel to reach each of the snapshots independently from the common graph.   In contrast, Kickstarter processes the snapshots sequentially, making it difficult to parallelize the processing.  In Table~\ref{parallel}, we show the time for the longest direct hop evaluation to reach any of the 50 snapshots.  Given a system with sufficient cores, this is an estimate of the overall run time of these embarrassingly parallel evaluations.  We can see that there is an opportunity to achieve speedups upwards of 2 orders of magnitude compared to Kickstarter. We note that it is also possible to parallelize the work sharing version of common graph, resulting in a more work efficient algorithm.



Figure~\ref{fig:breakdown} shows the breakdown of the execution time for the TTW graph both for KickStarter and \emph{CommonGraph} . As we can see, the \emph{CommonGraph} approach eliminates the mutation time for additions and deletions as well as the incremental deletion time. The incremental addition time for \emph{CommonGraph} is lower than the combined incremental addition and deletion time in KickStarter. Thus, we observe that benefits of \emph{CommonGraph} result from both reductions in computation cost and mutation cost.






==> incremental-algorithm.tex <==
\begin{algorithm*}[!t]
\begin{multicols}{2}
\begin{algorithmic}[1]

\State{\textbf{Inputs}: Snapshots; Additions; and Deletions.}
\State{Snapshots-- $G_1(V_1,E_1)$, $G_2(V_2,E_2)$, ... , $G_N(V_N,E_N)$; \\
Batches of Additions -- $\Delta_{G_1}^+$, $\Delta_{G_2}^+$, ... , $\Delta_{G_N}^+$; \\
Batches of Deletions -- $\Delta_{G_1}^-$, $\Delta_{G_2}^-$, ... , $\Delta_{G_N}^-$;}
\State{\textbf{Output}: $TG\;$ \& $\;Tree$ (Minimum Cost Schedule).}

  
\Function{Incremental Computation}{}

\EndFunction
\Statex{}

%\end{small}
\end{algorithmic}
\end{multicols}
\caption{Incremental algorithm}
\label{algo:incremental}
\end{algorithm*}

==> introduction.tex <==
%\vspace{0.05in}
\section{Introduction}
%\vspace{-0.075in}
%Graph analytics are important
Analyses on large graphs are an increasingly important computational workload as graph analytics is employed in many domains -- social networks~\cite{pk,tension,social,safety,higgstwitter}, web graphs~\cite{webmap}, brain networks~\cite{brain} and others -- to uncover insights by mining high volumes of connected data.  
 %Unlike traditional relational analytics that are based on ``one-to-one" or ``one-to-many" relationships, graph analytics  make it possible to ask more complex questions by exploring the ``many-to-many" relationships in graph data~\cite{graph}.  
 Due to the iterative nature of many graph analytics workloads, repeated passes over the graph are required until the algorithm converges to a stable solution. Since real-world graphs can be very large (e.g., \textsf{YahooWeb} has 1.4 billion vertices and 6.6 billion edges), iterative graph analytics workloads are highly memory-intensive. There has been significant interest in developing scalable and efficient graph analytics systems. Some examples of such systems are   Ligra~\cite{ligra}, Galois~\cite{galois}, GraphChi~\cite{graphchi}, GridGraph~\cite{gridgraph}, GraphLab~\cite{graphlab}, GraphX~\cite{graphx},  and PowerGraph~\cite{powergraph}.
 
 %Dynamic graph analytics 
 Graphs are often dynamic, with edges and vertices being added or removed over time~\cite{besta-21}. There are two broad classes of analyses on dynamic graphs: (1) \emph{Streaming graph analytics}: where results of a query are continuously updated as the graph continues to change because updates to it stream in over time; for example, we may want to maintain the shortest path to a destination as the traffic conditions change. Typically incremental algorithms are employed to update query results in response to graph changes and thus avoid recomputing the query from scratch~\cite{kickstarter,jetstream,kineograph,stinger,10.1145/2882903.2882950,graphbolt,tripoline}; and (2) \emph{Evolving graph analytics}: in this scenario, queries seek to answer questions about a dynamic graph as it evolves over longer time scales~\cite{tegra,chronos,kevaltaco}. Multiple snapshots of the graph are available in this scenario. Typically an evolving graph (EG) query seeks to \emph{track a graph property over a long time scale} by computing its value at different snapshots within the time window identified by the query. This makes the problem potentially significantly more computationally expensive than both traditional analytics on a static graph as well as streaming analytics on a changing graph. 
  
%Traditional approaches to evolving graphs and what is wrong with them
A straightforward approach to this problem is to apply the query to the individual snapshots independently; however, this approach has significant overheads since we end up solving the query independently on many different snapshots. Alternatively, another approach that has been used~\cite{risgraph,tegra} starts from the earliest snapshot and uses streaming to move from one snapshot to the next in sequence. While this approach results in significantly less work, provided that the number of changes between snapshots is not too large, it has a number of drawbacks. First, we show that for many algorithms the cost of edge deletions is very high; thus, performance benefits of the incremental algorithm are limited. Second, the solution moves between snapshots in sequence which limits opportunities for sharing query evaluation work among them.  
%\nael{I dont think the second point is true.  Arguably, streaming creates even more reuse as every earlier update (unless it is modified later) ends up being reused by remaining snapshots.  Its difficult to articulate the advantage of commongraph -- i think its more the fact that it is essentially "equidistant" from the different snapshots allowing us to approach them in parallel rather than sequentially by adding the right path. Rajiv: The problem with parallel argument is twofold -- we don't do anything in parallel; and the work that Keval published in TACO already does multiple snapshots in parallel while reusing results.} \nael{A thought perhaps for the future.  What if we go to the traffic example and an edge experiences a lot of short term fluctuation (traffic going up then going down).  Streaming will have to process all of those, while with commongraph we have only the last update to apply (I think) for each snapshot.  Maybe we need some kind of sampling that avoids the short term events in the evolving graph representation. Rajiv: Streaming does not have to process all the ups and downs, it can skip intervening changes -- it is done in batches any way which has the same effect. Also weight changes can be handled without deletions -- that is what Xizhe's current in progress paper is about so it is not a good scenario for this paper -- another thing is that in the traffic example we need answer to a particular destination -- point-to-point query-- which is different than this work.}
  
%Introduce our approach and algorithm at a high level
In this paper, we propose \emph{CommonGraph}, a new algorithm and system for efficiently evaluating an evolving graph query. \emph{CommonGraph} reduces the overhead of multiple evaluations by identifying the common subgraph that is shared by the multiple snapshots of interest. Specifically, we first process this common graph, sharing this overhead among all the snapshots, and then stream in additional edges that convert this common graph into each of the other snapshots. \emph{CommonGraph} is motivated by two key new insights: 
\begin{enumerate}\itemsep2pt
    \item \emph{Converting expensive deletions to additions.}  We show that the incremental cost of processing deletions is significantly greater than additions for an important class of algorithms that is monotonic (these are the algorithms supported by Kickstarter).%\nael{Please check the previous sentence} 
    Therefore, the \emph{CommonGraph} is designed to naturally convert all deletion operations into addition operations--we start with the common set of edges across a group of snapshots, and only have to add edges to reach any snapshot, eliminating the high overhead deletions. The overhead of graph mutation is also reduced with only additions; and
    
    \item \emph{Breaking the dependencies between incremental computations.} The addition of edges to reach any snapshot is an independent operation and thus, we can benefit from the efficient incremental additions algorithm for all snapshots. This makes possible a new structure, the \emph{Triangular Grid}, that enables further \emph{work sharing} among subsets of snapshots via reuse of the edge additions shared by them.  
\end{enumerate}
  



\vspace{0.05in}
%Explain a little about the implementation
We implement \emph{CommonGraph} by extending the Kickstarter~\cite{kickstarter} system, a state of the art streaming graph framework; \emph{CommonGraph} is a general algorithmic idea that can be implemented within other frameworks as well.  We observe that the dynamic graph update process within kickstarter is extremely expensive, and, given the structure of \emph{CommonGraph} come up with a graph representation that adds the new edges without having to change the primary graph representation. This strategy also enables us to share the common changes naturally among multiple snapshots in a space efficient way.  This implementation enables us to compare \emph{CommonGraph} against the two baselines: computing the query on each snapshot; and streaming all the changes from the initial snapshot.
%using Kickstarter. 

\vspace{0.1in}
The key contributions of our work are as follows:
\begin{itemize}
    \item A new approach to evolving graphs analysis that avoids processing of expensive deletions by converting all graph updates to additions over the \emph{CommonGraph}, replaces expensive deletions by additions, and removes dependencies that enable work sharing among the snapshots.
    \item A new structure called {\em Triangular Grid} (TG) that exposes work sharing possibilities among the snapshots. We demonstrate that maximizing work sharing corresponds to solving the Steiner tree problem on the TG, enabling further optimization of evolving graph queries.
    %\emph{work sharing} among multiple snapshots, and reduces the overhead of performing graph mutations;
    \item A graph representation that avoids the need to mutate graphs and enables reuse of edges by snapshots that share them.
    \item We build the \emph{CommonGraph} that exploits the three ideas above to achieve speedups ranging between 1.38$\times$ and 8.17$\times$ over Kickstarter both by avoiding deletions and performing work sharing. Further speedups are also possible since the evaluations of the snapshots are highly parallelizable.    
\end{itemize}

%\textit{(a) Concurrent Query Evaluation.} Since both snapshots, $G_i$ and $G_{i+1}$, are available at the start, we can simultaneously evaluate the query on both. This motivates our first extension: using an integrated compacted version of both snapshots, the software will simultaneously process both versions concurrently.

%\textit{(b) Ordered Query Evaluation -- Forward vs. Backward Direction.} A query can be evaluated in either forward order (i.e., $G_i$ first) or backward order (i.e., $G_{i+1}$ first).

%\textit{\textbf{Forward Evaluation}}: Since $G_i$ + $\Delta^{i}_+$ - $\Delta^{i}_-$ $\rightarrow$ $G_{i+1}$, we can first evaluate the query $G_i$ and then for $\Delta^{i}_+$ additions and $\Delta^{i}_-$ deletions we incrementally evaluate query for $G_{i+1}$.
    
%\textit{\textbf{Backward Evaluation}}: Since $G_{i+1}$ - $\Delta^{i}_+$ + $\Delta^{i}_-$ $\rightarrow$ $G_i$, we can first evaluate the query on $G_{i+1}$ and then for $\Delta^{i}_+$ deletions and $\Delta^{i}_-$ additions we incrementally evaluate query for $G_i$.

%We  observe that processing deletions is many fold more expensive than processing additions. As a result, we would like to minimize the processing of deletions. Therefore, if $\Delta^{i}_+$ $\geq$ $\Delta^{i}_-$, then forward order is preferable, and if $\Delta^{i}_-$ $>$ $\Delta^{i}_+$, then the backward order is preferred.

%\textit{(c) Concurrent Additions-Only Evaluation.} Finally, we present an evaluation plan that combines \textit{concurrency} with incremental processing that involves \textit{only additions}. In particular, we will first evaluate the query on the \textit{common subgraph} of $G_i$ and $G_{i+1}$, say $G_c$, that contains edges that are present both in $G_i$ and $G_{i+1}$. Next we compute the query for $G_i$ and $G_{i+1}$ from $G_c$ concurrently. This is done by incrementally processing the additions of $\Delta^{i}_-$ to $G_c$ and separately $\Delta^{i}_+$ $+$ $\Delta^{i}_-$ to $G_c$ to obtain the results for $G_i$ and $G_{i+1}$ respectively. 
%Although we have considered only two snapshots in the above discussion, we will also extend the above ideas to a series of snapshots. Let us assume that we are interested in evaluating a query on a series of graph snapshots $G_0, G_1, \cdots G_n$. Here $G_c$ can be the common subgraph that has all the edges common to all the snapshots $G_0, G_1, \cdots G_n$. Then via additions-only incremental algorithm, using the results of $G_c$, results for $G_0, G_1, \cdots G_n$ can be simultaneously computed.




==> related.tex <==

\section{Related Work}
In this section we summarize the existing dynamic graph systems and accelerators that aim at providing flexible graph storage and fast incremental concurrent graph querying.

%\vspace{-0.1in}
\subsection{Evolving \& Streaming Graphs Frameworks}
Among the most recent works on rapid analysis of evolving graphs are RisGraph~\cite{feng2021risgraph} and Tegra~\cite{tegra}. RisGraph achieves impressive query evaluation speeds by developing a new data structure to support fast edge insertions and deletions. However, this is achieved at the expense of 3.25$\times$ to 3.38$\times$ increased memory costs via precomputed indexes that are necessary to support both fast insertions and deletions. Tegra~\cite{tegra} provides a novel API for performing ad-hoc queries on arbitrary time windows of the graph. It accelerates query evaluation using a compact in-memory representation for both graph and intermediate computation state. Both RisGraph and Tegra leverage existing algorithms developed for streaming systems to support incremental computation for handling edge additions and deletions. Other storage systems to support evolving and streaming graphs include GraphOne~\cite{kumar2020graphone} and Aspen~\cite{aspen} while systems that amortize the cost of memory accesses and computation include Chronos~\cite{chronos} and FA+PA~\cite{kevaltaco}.

A number of systems for streaming graphs have been proposed. These algorithms maintain a single version of the graph and a standing query's results that are incrementally updated when a batch of updates are applied to the graph. The focus of these works is on incremental computation, i.e. how to efficiently update query results. Early streaming systems (such as Kineograph~\cite{10.1145/2168836.2168846}, Naiad~\cite{naiad},  Tornado~\cite{10.1145/2882903.2882950} and Tripoline~\cite{tripoline}) only support incremental computations for edge additions while more recent systems (such as
Kickstarter~\cite{kickstarter} and GraphBolt~\cite{graphbolt}) also support edge deletions. 

Note that even though many of the above evolving and streaming systems support both edge additions and deletions, they pay a high cost for supporting deletions, as we showed in the comparison to Kickstarter. \emph{CommonGraph} is the first system to convert deletions into additions for evolving graph analysis and thus reduce the cost of graph mutation as well as incremental computation (via work sharing) significantly.


%\nael{Single sentence unclear summary of the related work in the paragaraph below.  You should explain why the idea is important and how common graph is either orthogonal or has some advantages at least in some places compared to it.}
%Tegra: for graph incremental computation and snapshots flexible storage. However, these proposed solutions suffered from expensive graph mutation overhead and lack of concurrently queries supports, also, the incremental algorithm utilized in those system lack of the ability to remove redundant computation in the evolving-graph workloads.
%Risgraph targets efficient streaming for evolving graphs\cite{feng2021risgraph}.  It proposes a new  data structure that apriori tracks the footprint of an edge deletion, moving that overhead to be offline.  It also introduces a domain-specific concurrency control mechanism for real-time dynamic graph processing.  Unfortunately, the new data structure requires 3.5x memory overhead, making it impractical for large graphs.
%GraphOne\cite{kumar2020graphone} developed a high-performance data storage system for dynamic graph mutation.\nael{Say more} GraphInc\cite{cai2012facilitating},  GraphU\cite{10.1145/3267809.3267811} processes new graph snapshots by using pre-calculation with pre-processed updates.\nael{And?} 
%To handle multi-snapshots concurrently, Aspen\cite{aspen} developed compressed tree structure to store multi-version graph for parallel execution.  
%Chronons~\cite{chronos} and FA+PA divided snapshots into different batches for reducing fetch and process cost purpose.\nael{Unclear} DZiG\cite{10.1145/3447786.3456230} proposed DelZero-port to query multiple snapshots concurrently.\nael{and?} SAMS\cite{then2017automatic} replace algorithm computation by accessing shared graph data to process graph queries.   


%\vspace{-0.05in}
\subsection{GPUs and Other Accelerators}

Recent works have begun to exploit accelerators to speedup up graph algorithms. Much of this work is aimed at static graphs (e.g.,  Gunrock~\cite{gunrock}, CuSha~\cite{cusha,cusha2},Tigr~\cite{tigr}, Subway~\cite{subway} etc.) and the problem addressed is to map irregular graph computation to regular GPU architectures. Specialized graph accelerators have also been developed for both static graphs~\cite{graphpulse,polygraph,GraphPIM,Tesseract} and streaming graphs~\cite{jetstream,inputk,10.1145/3470496.3527409}. Some recent works have begun to support dynamic graphs in accelerators such as GraSu~\cite{wang2021grasu}. However, to our knowledge, no work has been done to exploit single accelerators to address evolving graph analysis. We expect that the tremendous memory and computational demands of evolving graphs will require development of multi-accelerator systems.

%Limited works have looked at supporting dynamic graphs on GPUs.  Several efforts including cuSTINGER\cite{green2016custinger}, Hornet\cite{busato2018hornet}, aimGraph\cite{winter2017autonomous} faimGraph\cite{winter2018faimgraph} propose different dynamic data structures for GPU. For the purpose of efficiently executing graph updates, GPMA\cite{10.14778/3151113.3151122} proposes a dynamic graph system, designed to fully utilize the high performance of GPU.\nael{How? What is the insight?}  While these works represent significant advances in supporting dynamic graph analysis on GPUs, they suffer from high data access overhead and low memory bandwidth utilization ratio due to the irregular access patterns in dynamic graph processing.  For static graphs, some prior work targets improving the memory access behavior in graph processing, but these ideas are not as effective for dynamic graphs.\nael{Can you cite these papers?  Why are they ineffective for dynamic graphs?}
%\subsection{Graph Accelerators for dynamic graph processing}
%Template based graph accelerators process hundreds of vertices in parallel to mask long memory latency. They use hardware supported primitives for synchronization.\nael{Cite these accelerators?  What do you mean by template based?} Jetstream\cite{jetstream} and GraphPulse\cite{graphpulse} supports both accumulative and monotonic graph algorithms updates query by extends a recently proposed event-based accelerator for graph workloads, but they do not support control to multi-snapshots to enable evolving graph processing. GraSu\cite{wang2021grasu} uses a differential data management to reserve high degree vertices based on spatial similarity for fast graph mutation. TDgraph\cite{10.1145/3470496.3527409} utilizes many-core processors to achieve high performance processing of streaming graphs based on an efficient topology-driven incremental execution approach.  We are not aware of any accelerators that can support multi-version operation and therefore Evolving Graphs.

% Swarm proposes a custom architecture for speculative execution to increase parallelism; however, the memory inefficiencies persist. Graphicionado is a pipelined hardware architecture designed to optimize conventional vertex-centric graph models using a fast temporary memory space. The architecture improves locality using a shadow memory space in the on-chip memory for vertex property updates. Hardware accelerators proposed by Zhou et al. exploit an approach of storing contributions temporarily to memory and combining them using hardware support when possible in an edge-centric model. However, for a large number of edges there is a substantial increase in number of random memory accesses needed for writing to temporary memory bins and the small sized combination window can only achieve limited memory access reduction. 

% \subsection{PIM-Based solution}
% Several researchers use the concept of processing-in-memory to decrease memory access latency and thus increase performance. Tesseract proposes an architecture that implements simplified general purpose processing cores in the logic layer of a 3D stacked memory. GraphPIM replaces atomic operations in the processor with atomic operation capabilities in the proposed Hybrid Memory Cube (HMC) 2.0 specification to achieve low latency execution of atomic operations. Other PIM based solution looks at robust partitioning and cross-communication approaches to fit large graphs in limited 3D stacked memory. Our accelerator has potential advantage on processing-in-memory platforms too. Event coalescing for graph slices not residing on the accelerator can be implemented directly in memory. 

% \subsection{GPU-based dynamic graph system}
% \vspace{0.1in}
% \subsection{FPGA-based dynamic graph system}
% \vspace{0.1in}
% \subsection{Dynamic graph accelerator}
% \vspace{0.1in}
% \subsection{Static graph system}


==> system.tex <==
\section{CommonGraph System}

In this section we discuss our system design and implementation for processing evolving graphs using \emph{CommonGraph} algorithms. We first present an overview of the framework and then describe the core processing engine in more detail.

%of the illustrate the multi-snapshots system construction and graph queries over series of snapshots.
%\vspace{-0.02in}


\subsection{Framework overview}
% Unlike Aspen\cite{aspen}, Risgraph\cite{risgraph} or Tegra\cite{tegra}, which use compressed tree structure for version-control, 


% to.  We can then initialize the $\Delta_+$ or $\Delta_-$ edge lists from the update edge list to create the Triangular Grid structure using Algorithm~\ref{algo:tree_construction}. 

% For the common graph storage, we follow the format used in Ligra~\cite{ligra}, which represents the in-edges and out-edges as arrays, partitioned by the source vertices and each storing the target vertices. 
% For weighted graph, the weights are interleaved with the destination of the edge with the goal of improving cache locality on edge accesses.
% With respect to the $\Delta$ edges which represent the deletions and additions between different snapshots, our framework supports both CSR format and edge list format.  
% The edge list format records both the source and destination of the edges.  The edge list is used when the batch sizes are smaller then the maximum number of vertices, in which case the edge list format is more storage compact. However, a downside of using edge lists is that when we conduct graph queries over different snapshots, the overhead increases since traversing the edge list has higher time complexity over traversing CSR format storage.  
% An overhead comparison of CSR vs. edge list format can be seen in Figure.\nael{Which figure?}

\begin{table}[!b]
\captionsetup{justification=centering}
\caption{Common graph main primitives for query \\ computation and graph update.} %\nael{This Table needs some work to provide some structure or intuition into why these are the right primitives. Do we need to show all these primitives?  Formatting is also off.  Could consider omitting.}
\label{API}
\vspace{-0.05in}
%\small
\centering
\begin{tabular}{|l|l|} \hline
% Coarse grain primitive
% & Description
% \\ \hline \hline
Version control API
&\thead{Description} 
\\ \hline \hline
% algorithm(Snapshots[size]) & return query results as arrays\\ \hline
get$\_$version(number) & \thead{Retrieve a snapshot} \\ \hline
diff(snapshot, snapshot)& \thead{Identifies difference between \\ two snapshots} \\ \hline
% abs$\_$diff(snapshot) &  \thead{identifies difference between \\ common graph and a snapshot} \\ \hline 
new$\_$version($\Delta_+$, $\Delta_-$) & \thead{Create a new snapshot and \\update common graph}\\ \hline\hline
Query API & \thead{API function} \\ \hline \hline

% common$\_$push($\&$vertex$\_$id) & \thead{push info to neighbors \\among common graph}  \\ \hline
% $\Delta\_$push($\&$vertex$\_$id, $\Delta$) &\thead{push operation}  \\ \hline 
edge$\_$function(edge) & \thead{Algorithm specific edge function}\\ \hline
schedule(vertex$\_$id, mode) & \thead{Schedule active vertex} \\ \hline
update(vertex$\_$id) & \thead{Atomic update function} \\ \hline
% $SSSP(Snapshots[size]) \hookrightarrow vertex\_array[size]$ \\ \hline
% $SSWP(Snapshots[size]) \hookrightarrow vertex\_array[size]$ \\ \hline
% $SSNP(Snapshots[size]) \hookrightarrow vertex\_array[size]$ \\ \hline
% $Viterbi(Snapshots[size]) \hookrightarrow vertex\_array[size]$ \\ \hline
\end{tabular}
%\vspace{-0.25in}
\end{table}

The framework consists of the storage and memory representation of the evolving graphs, as well as the set of primitives to manage the storage and the version control of the snapshots in memory during execution.  We discuss these aspects of the framework next.

We use the common graph as the basis for storing the graph as a series of common graphs for each range of snapshots as well as the set of edges in the Triangular Grid for each of them. Thus, there is a minimal cost for generating common graphs while the updates are stored as sets of $\Delta$ edges corresponding to the Triangular Grid edges. For Kickstarter~\cite{kickstarter}, we use its storage format based on Ligra~\cite{ligra}.

The key feature of the data structures that we use to support evolving graphs is that we avoid the cost of updates to the graph as it evolves. % he major difference between common graph systems and other traditional dynamic graph system is our version control does not require any mutation or any other changes to the original graph. 
As discussed in Section~\ref{section3}, the common graph and $\Delta$ edges are stored separately, and different versions of the graph are reached by including different subsets of the $\Delta$ edges as specified by the TG.   The representation is space optimal as each edge in the system only gets represented once.  In addition to avoiding expensive mutations, this organization also significantly reduces both memory footprint and memory access overheads.
%As discussed in Section \ref{section3}, we applied "common + Triangular Grid" strategy for disambiguation of the computation of the different snapshots. %The key idea is we only keep edges that are shared among all the snapshots in a common graph  structure. In addition, 
%All the streaming edge lists are represented outside of the common graph as nodes in TG with compressed sparse row (CSR) format.  
To access the graph, we support the primitives shown in Table~\ref{API}.  These  primitives are used to retrieve a snapshot or find the difference between snapshots. The overhead in querying a snapshot is much lower than that in Aspen~\cite{aspen}, which is a multi-version storage system for evolving graphs; the overhead for Aspen has up to 2$\times$ overhead than Ligra+ on static graphs.  

When a new snapshots are to be created by a stream of batches, the system uses the batches to update the common graph and the TG. Specifically, the new edges (both the additions and deletions) will be removed from the common graph and additional nodes representing the new snapshot will be added to the TG. % \nael{Maybe show a diagram?}

%\begin{figure}[!b]
 %   \vspace{-0.025in}
  %  \centering
   % \includegraphics[width=1.0\columnwidth]{diagrams/section4.png}
%    \caption{High level overview for graph query engine}\nael{Can you connect the bit scheduler to the output of the analysis to create the execution loop?  Right now its not clear where the refresh bit scheduler arrow comes from.}
 %   \label{fig:queries highlevel}
  %      \vspace{-0.125in}
%\end{figure}
%\subsection{Algorithm API}

% Systems like Tegra~\cite{tegra} and Risgraph~\cite{risgraph} provide users with streaming graph construction APIs, supporting primitives such as insertion, deletion and get version.  The goal of these systems is to support fast mutation of the graph.  In contrast, our system targets at providing high-performance graph queries over a series of different snapshots.  As a result, we designed the system to use a different set of primitives that are illustrated in Table \ref{API}.   In a typical scenario, users provide the query algorithm and the snapshot details and the system generates the query values at each of the snapshots.

\begin{algorithm}
% \vspace{-0.25in}
\begin{algorithmic}[1]

\State{\textbf{Inputs}: common graph; streaming batches, query algorithm;}

\State{\textbf{Output}: Query result $\hookrightarrow$ vertex$\_$value$\_$array[].}
\Function{Incremental Computation}{}
% \State{$\Delta\_$ = abs$\_$diff(common$\_$graph, graph$\_$query);}
\For{edge in streaming batches}
\If{\textcolor{red}{edge$\_$function}(edge) == True;}
\State{\textcolor{red}{update}(destination);}
\State{\textcolor{red}{schedule}(dst, mode);}
\EndIf
\EndFor
\While {\textbf{scheduler} is not empty}
\For{vertex in \textbf{scheduler} }
% \State{push(vertex);} \Comment{vertex are pushed among both common graph and streaming batches}
% \State{$\Delta\_$push(vertex);}
\For{edges $\in$ \textbf{common graph+update batch}}
\If{\textcolor{red}{edge$\_$function}(edge) == True;}
\State{\textcolor{red}{schedule}(vertex, mode);}
\EndIf
\EndFor

\EndFor
\EndWhile
\EndFunction
% \Statex{}


\end{algorithmic}

\caption{Mutation-Free Incremental Algorithm}
\label{algo:incremental}
\end{algorithm}


\subsection{Execution Engine}
% \vspace{-0.125in}

% To support both initial computation on the common graph, and incremental computation as edges are added, we followed the vertex-centric model supported by Ligra.  We do not use the pull operation in hybrid mode supported by Ligra. The computation on the common graph generates a high number of updates compared to the incremental update phase of the computation; we use a bit scheduler structure for iterative computation which is able to perform synchronization and asynchronous vertex update efficiently.%\nael{What is the bit scheduler?  Why is it efficient?  How does it relate to the difference in computation density?}  

The system executes a query targeting multiple snapshots in two steps: \emph{a scheduling phase}; and \emph{a computation phase}. The scheduler derives the query execution plan following Algorithm~\ref{algo:tree_construction}, this step is not needed for direct hop. The query execution phase is divided to two parts: initial computation of the query on the common graph and incremental update to add the batches to reach the next graph, and eventually all the snapshots. In the initial stage, computation happens on the common graph only, with active vertices pushing information to neighbors. The computation iterates till the graph stabilizes. For the second phase, we extend the Kickstarter streaming algorithm as shown in Algorithm~\ref{algo:incremental}.   Specifically, the system first starts with streaming batches (lines 4-9), the destination vertices are updated and scheduled based on the edge function. Next, the scheduled vertices repeatedly push updates to their outgoing neighbors and new vertices are scheduled and updated (Algorithm~\ref{algo:incremental}, lines 10-18). The steps in the algorithm shown in red are APIs for programming the engine.

A major difference between common graph engine and other streaming engines is it takes a graph with batches of streaming edges as input instead of doing computation on just single version. The edge function in Table~\ref{API} is applied both on common graph and streaming batches. This strategy avoids expensive graph mutation operation with reasonable overhead.% as shown in Table~\ref{overhead}.
%\nael{Can you talk about the differences from Kickstarter?  It sounds identical to kickstarter with commongraph being the initial snapshot} % The process is shown in figure \ref{fig:queries highlevel}.

% More specifically, the bit scheduler design follows the scheduling policy proposed by GraphChi~\cite{graphchi}, which represents the current set of active vertices as a bit-array.   When we enable the asynchronous mode during incremental update, the vertices that are updated are scheduled in the current iteration. This scheduling approach is helpful for small batch incremental computation.   More details are illustrated in algorithm \ref{algo:incremental}.


%\subsection{Graph queries}
% After the framework is constructed, users can provide a series of snapshots' number and query algorithms as the inputs to the system. The system will generate the output represented as vertex arrays for different snapshots.
% Graph query execution is divided into three steps: query evaluation schedules, common graph computation and incremental computation.   Both query evaluation schedules and common graph computation can be generated offline.  The schedules can be calculated by batch sizes \nael{This is unclear.} while the common graph can be pre-generated offline or even used directly as the storage format. For incremental computation, the evaluation iterates through activation, vertex scheduling and iterative computation, as illustrated in Figure \ref{fig:queries highlevel}.  For example to reach the leaf node snapshots from the common graph, we take both the common graph vertex array and all the $\Delta$ edge arrays as input. Using the $\Delta$ edges, we activate the vertices whose values got affected by the streaming batches and add the affected vertices to the scheduler list. After all the $\Delta$ edges are traversed and vertices are scheduled, we perform the push operation among both common graph and streaming batches to generate new scheduler lists for the next iteration, this process will repeat until the vertex values stabilize.

%\nael{Overall, this section is not so clear.   Chao, lets discuss when you have time.}
\subsection{Scheduler design}
Scheduler referenced in Algorithm~\ref{algo:incremental} on lines 10-11 incorporates another policy in our system. The key idea is to switch between synchronous and asynchronous mode. For large streaming batch, the scheduler will work in synchronous mode, and vertex updates will take effective in next iteration. For a small streaming batch, the scheduler is set to asynchronous mode and updated vertex value will be available in the current iteration. 
%\subsection{Memory Footprint}

% The \emph{CommonGraph} system uses an initial graph and the sets of edge additions to move between the difference snapshots. The edge lists are stored in CSR format for data locality. The vertex property arrays are kept with the vertex id as the horizontal coordinate and the version number as the vertical coordinate. To support concurrent execution on multiple snapshots, \emph{CommonGraph} holds multiple active vertex arrays. Since it does not replicate any information, the memory utilization is similar in  size to streaming graph system like Kickstarter\cite{kickstarter} or RisGraph\cite{risgraph}.

==> usermacros.tex <==
\newcommand{\graphpulse}{\textsf{{GraphPulse}}\xspace}

\newcommand{\jetstream}{\textsf{{JetStream}}\xspace}

\newcommand{\ED}{{event-driven}\xspace}

\newcommand{\identity}{\textit{Identity}\xspace}

\newcommand{\shafi}[1]{\textcolor{teal}{#1}}

% \newcommand{\nael}[1]{\textcolor{blue}{Nael: #1}}
\newcommand{\nael}[1]{}


\newcommand{\circledstep}[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {#1}}}}


% \newcommand{\change}[1]{\textcolor{teal}{Changed here: #1}}

% \newcommand{\factcheck}[1]{\textcolor{orange}{#1}}
\newcommand{\factcheck}[1]{{#1}}

\newcommand{\cut}[1]{{ }}

\newcommand{\replace}[2]{\sout{#1} \textcolor{purple}{#2}}
\newcommand{\add}[1]{\textcolor{purple}{#1}}
\newcommand{\delete}[1]{\textcolor{purple}{\sout{#1}}}
\newcommand{\revise}[1]{\hl{#1}}
%\newcommand{\stash}[2]{\textcolor{olive}{#1}}
\newcommand{\stash}[2]{#2}

\newcommand{\graycell}{\cellcolor[rgb]{ .851,  .851,  .851}}

% \setlength {\marginparwidth }{2cm}


\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\soulregister\cite7
\soulregister\ref7
\soulregister\jetstream7
\soulregister\graphpulse7
\soulregister\textsf7
\soulregister\emph7
